Universality Laws for High-Dimensional Learning with Random Features

We prove a universality theorem for learning with random features. Our result shows that, in terms of training and generalization errors, a random feature model with a nonlinear activation function is asymptotically equivalent to a surrogate linear Gaussian model with a matching covariance matrix. This settles a so-called Gaussian equivalence conjecture based on which several recent papers develop their results. Our method for proving the universality theorem builds on the classical Lindeberg approach. Major ingredients of the proof include a leave-one-out analysis for the optimization problem associated with the training process and a central limit theorem, obtained via Stein's method, for weakly correlated random variables.

==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/abstract.tex <==
%!TEX root = get_kernel.tex

\begin{abstract}
We prove a universality theorem for learning with random features. Our result shows that, in terms of training and generalization errors, a random feature model with a nonlinear activation function is asymptotically equivalent to a surrogate linear Gaussian model with a matching covariance matrix. This settles a so-called Gaussian equivalence conjecture based on which several recent papers develop their results. Our method for proving the universality theorem builds on the classical Lindeberg approach. Major ingredients of the proof include a leave-one-out analysis for the optimization problem associated with the training process and a central limit theorem, obtained via Stein's method, for weakly correlated random variables.
\end{abstract} 

==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/clt_new.tex <==
%!TEX root = get_kernel.tex
\section{A Central Limit Theorem for the Feature Model}
\label{sec:CLT}

In this section, we prove a central limit theorem (CLT) related to the nonlinear feature model. Let
\begin{equation}\label{eq:ab_vec}
\va = \kernel(\fmtx\tran \cvec) \quad \text{and} \quad \vb = \mu_1 \fmtx\tran \cvec+ \mu_2 \vz,
\end{equation}
where $\cvec \sim \mathcal{N}(0, \mI_d)$ and $\vz \sim \mathcal{N}(0, \mI_p)$ are two independent Gaussian vectors, $\fmtx = [\vf_1, \ldots, \vf_p]$ is a collection feature vectors in $\R^d$, and $\mu_1, \mu_2$ are constants as defined in \eref{mu_constants}. Given the teacher vector $\sgl$ in \eref{teacher} and a second vector $\wvv \in \R^{p}$, we show that
\begin{equation}\label{eq:CLT_approx}
\big(\scp{\va\tran \wvv}, \cvec\tran \sgl\big) \overset{\text{Law}}{\approx} \big(\scp{\vb\tran \wvv}, \cvec\tran \sgl\big)
\end{equation}
as $p \to \infty$. Here, we consider the setting where $\wvv, \sgl$ and the feature vectors are all \emph{deterministic}, and the only sources of randomness come from $\cvec$ and $\vz$. Thus, the right-hand side of \eref{CLT_approx} are just two jointly Gaussian random variables. 
\textcolor[rgb]{0.00,0.00,0.00}{
CLT in the form of \eref{CLT_approx} was first studied and proved in \cite{Goldt2020Gaussian} (see our discussions in Section \ref{subsec:relatedwork} and Remark \ref{rem:CLT} below).}
It will be useful in bounding the term $\Delta_\text{CLT}$ in \eqref{eq:Phi_k_decomp_2}, a critical step in our application of the Lindeberg method. It also plays an important role in our proof of Proposition~\ref{prop:gen}, where we establish the universality of the generalization error.

To state the theorem, we first need to put some restrictions on the feature vectors and the teacher vector $\sgl$. Let $\fvec_0 \bydef \sgl$, and let $\delta_{ij}$ denote the Kronecker delta function. We assume that
\begin{equation}\label{eq:BP}
\max_{0 \le i, j \le p} \abs{\vf_i\tran \vf_j - \delta_{ij}} \le \frac{\BP}{\sqrt{p}}
\end{equation}
for some $\BP = \mathcal{O}(p^{1/8 - \gamma})$ and $\gamma > 0$. Moreover,
\begin{equation}\label{eq:fnorm}
\norm{\fmtx} \le \polylog p.
\end{equation}
Note that, for the random feature vectors considered in this paper [see Assumption~\ref{a:feature} and the admissible condition in \eref{def_setA1}], the upper bound $\BP$ can actually be as small as $\polylog p$, and the spectral norm $\norm{\fmtx}$ can be set to be of $\mathcal{O}(1)$. However, since we believe that the central limit theorem could be of independent interest in other problems beyond this paper, we are going to prove it under the more relaxed assumption in \eref{BP}.

\begin{thm}\label{thm:CLT_general}
Suppose that the feature vectors satisfy \eref{BP} and \eref{fnorm}, and the activation function $\sigma(x)$ satisfies the conditions in Assumption~\ref{a:kernel}. Let $\set{\btest_p(x; s)}$ be a sequence of two-dimensional test functions that are differentiable with respect to $x$. Moreover, for each $p$,
\begin{equation}\label{eq:btest_condition}
\max\set{ \abs{\btest_p(x, s)}, \abs{\btest'_p(x, s)}} \le B_p(s)(1 + \abs{x}^K)
\end{equation}
for some constant $K \ge 1$ and some function $B_p(s)$. For any fixed vectors $\wvv \in \R^p$ and $\sgl \in \R^d$ with $\norm{\sgl} = 1$, it holds that
\begin{equation}\label{eq:CLT_general}
\begin{aligned}
    &\Big|\E \btest_p\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)-\E \btest_p\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)\Big| \\
    &\hspace{6.5em}\le\frac{[\E B_p^4(z)]^{1/4}P({\wvv}, \BP)\polylog p}{\sqrt{p}},
\end{aligned}
\end{equation}
where $z\sim\mathcal{N}(0,1)$ and $P({\wvv}, \BP) = [1 + \norm{\wvv}_\infty (1+\BPf)][1 + (\scp\norm{\wvv})^{2K+1}]/\mu_2^2$.
\end{thm}
\begin{rem}
\label{rem:CLT}
We prove this theorem in \sref{CLT_general}, after first establishing two lemmas in \sref{CLT_1D} and \sref{CLT_cond}. 
\textcolor[rgb]{0.00,0.00,0.00}{As mentioned in Section \ref{subsec:relatedwork}},
a CLT in the form of \eref{CLT_approx} was first proved in \cite{Goldt2020Gaussian}. In principle, we could have adapted the proof there. However, as the CLT needs to be integrated with other components of our proof in \sref{Proof-Sketch}, we find it more convenient to derive an alternative proof, with a bound in \eref{CLT_general} that brings forth the explicit dependence of the approximation error on the $\ell_\infty$ norm of $\wvv$. The emphasis on $\norm{\wvv}_\infty$ is an important point. Later, when the CLT is applied [see \eref{Phi_k_decomp_2}], the vector $\wvv$ in \eref{CLT_general} will be $\loowt{\bs k}$, \emph{i.e.}, the leave-one-out optimal solution of \eqref{eq:LOO_objctive_function}. Showing that $\norm{\loowt{\bs k}}_\infty$ is bounded with high probability turns out to be a nontrivial challenge (see Lemma~\ref{lem:loowt_l_infty_bd} and Proposition~\ref{prop:wt_bnd}). 

The settings of the CLT shown in \cite{Goldt2020Gaussian} are also somewhat different from ours. On the one hand, the one in \cite{Goldt2020Gaussian} is more general in that it does not require the nonlinear activation function $\kernel(x)$ to be an odd function. On the other hand, Theorem~\ref{thm:CLT_general} is more relaxed in terms of the test function $\btest(x; s)$, which only needs to be differentiable with respect to the first variable $x$. In addition, we further relax this restriction in \sref{CLT_disc}, where a characterization similar to \eref{CLT_general} is given for piecewise differentiable test functions, at the cost of a slower decay rate than the right-hand side of \eref{CLT_general}. This extension will be needed when we study the universality of the generalization error in \eref{gen_err}. Finally, the new proof technique here, based on Stein's method \cite{stein1972bound,barbour2005introduction}, might be of interest in its own right.
\end{rem}



%We also note that a similar CLT result was established in a recent work \cite{Goldt2020Gaussian}. Our results differ and complement each other in number of ways: (1) In terms of proof techniques, we use Stein's method \cite{stein1972bound,barbour2005introduction} to establish the central limit theorem, while \cite{Goldt2020Gaussian} is based on Lindeberg's approach. (2) Theorem \ref{thm:CLT_general} in the current paper holds when the random feature matrix $\fmtx$ satisfies $\fvec_{i}\tran\fvec_{j}= \mathcal{O}(p^{-3/8-\gamma})$ for $i\neq j$ [c.f. \eqref{eq:BP}], which implies that $\sum_{i\neq j}(\fvec_{i}\tran\fvec_{j})^4 = \mathcal{O}(p^{1/2-4\gamma})$. This regime is not covered by \cite[Theorem 2]{Goldt2020Gaussian}, which requires that $\sum_{i\neq j}(\fvec_{i}\tran\fvec_{j})^4 = \mathcal{O}(1)$.


\subsection{A Reduced Form of Theorem~\ref{thm:CLT_general}}
\label{sec:CLT_1D}


\begin{lem}\label{lem:CLT_1D}
Consider a sequence of activation functions $\set{\kernel_p(x)}$ and differentiable test functions $\set{\btest_p(x)}$ such that, for every $p$,
\begin{enumerate}
\item $\kernel_p(x)$ is an odd function;
\item $\max\set{\norm{\sigma'_p(x)}_\infty, \norm{\sigma''_p(x)}_\infty, \norm{\sigma'''_p(x)}_\infty} \le \polylog p$;
\item $\kernel_p(x)$ is compactly supported. Specifically, there is some threshold $\tau_p \le \polylog p$ such that $\kernel_p(x) = 0$ for all $\abs{x} \ge \tau_p$;
\item $\max\set{\norm{\btest_p(x)}_\infty, \norm{\btest'_p(x)}_\infty} \le B_p$ for some $B_p < \infty$.
\end{enumerate}
For any fixed vector $\wvv \in \R^p$, it holds that
\begin{equation}\label{eq:CLT_1D}
\Big|\E \btest_p\Big(\frac{\va\tran \wvv}{\sqrt{p}}\Big)-\E \btest_p\Big(\frac{\vb\tran \wvv}{\sqrt{p}}\Big)\Big|\le \frac{B_p(1 + \BPf) \norm{\wvv}_\infty \polylog p }{\mu_{2,p}^2\sqrt{p}}.
\end{equation}
Here, $\va = \kernel(\fmtx\tran \cvec)$ and $\vb = \mu_{1,p} \fmtx\tran \cvec+ \mu_{2,p} \vz$, where $\cvec \sim \mathcal{N}(0, \mI_d)$ and $\vz \sim \mathcal{N}(0, \mI_p)$ are two independent Gaussian vectors, $\fmtx = [\vf_1, \vf_2, \ldots, \vf_p]$ is a collection of feature vectors satisfying \eref{BP} and \eref{fnorm}, and
\begin{equation}\label{eq:mu_12p}
\mu_{1, p} = \EE[z\sigma_p(z)], \qquad  \quad \mu_{2, p} = \sqrt{\EE \sigma^2_p(z) - \mu_{1, p}^2},
\end{equation}
with $z \sim \mathcal{N}(0, 1)$.
\end{lem}
\begin{rem}
Lemma~\ref{lem:CLT_1D} is essentially a reduced form of Theorem~\ref{thm:CLT_general}. The characterization in \eref{CLT_1D} guarantees that $\frac{\va\tran \wvv}{\sqrt{p}}$ has an asymptotical Gaussian law, whereas \eref{CLT_general} needs to consider the joint distribution of $\frac{\va\tran \wvv}{\sqrt{p}}$ and $\cvec\tran \sgl$. Moreover, Lemma~\ref{lem:CLT_1D} puts some further constraints on $\sigma_p(x)$ and $\btest_p(x)$, requiring the former to have compact supports and the latter to be bounded and to have bounded derivatives.
\end{rem}


\begin{proof}
To lighten the notation in the proof, we will omit the subscript $p$ in $\sigma_p(x)$ and $\btest_p(x)$. Also note that, if $\norm{\wvv} = 0$, the left-hand side of \eref{CLT_1D} is $0$; if $\mu_{2, p} = 0$, the right-hand side is $\infty$. In either case, \eref{CLT_1D} holds trivially. Therefore, we assume $\norm{\wvv} > 0$ and $\mu_{2, p} > 0$ in what follows.

Our proof is based on Stein's method \cite{stein1972bound,Chen2011normal}. We start by observing that $\frac{\vb\tran \wvv}{\sqrt{p}}$ is a Gaussian random variable with zero mean and variance
\begin{equation}\label{eq:nu}
\nu^2\bydef \wvv\tran \mSig_b \wvv/p \quad \text{where} \quad \mSig_b \bydef \mu_{1, p}^2 \fmtx\tran \fmtx + \mu_{2, p}^2 \mI.
\end{equation}
It follows that we can rewrite the left-hand side of \eref{CLT_1D} as
\begin{equation}\label{eq:CLT_1Da}
\Big|\E \btest\Big(\frac{\va\tran \wvv}{\sqrt{p}}\Big)-\E \btest\Big(\frac{\vb\tran \wvv}{\sqrt{p}}\Big)\Big| =
\Big|\E \btest\Big(\nu\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big)-\E \btest(\nu z)\Big|
\end{equation}
for $z \sim \mathcal{N}(0, 1)$. Next, we introduce the following ``Stein transform'':
\[
\bts(x)\bydef e^{\frac{x^{2}}{2}}\int_{-\infty}^{x}e^{-\frac{y^{2}}{2}}\left[\btest\left(\nu y\right)-\E \btest\left(\nu z\right)\right]dy.
\]
Key to Stein's method is the following identity
\begin{equation}
\bts'(x)-x\bts(x)=\btest\left(\nu x\right)-\E \btest\left(\nu z\right),\label{eq:stein_identity}
\end{equation}
which can be directly verified from the definition of $\bts(x)$. Moreover, since $\norm{\btest'(x)}_\infty \le B_p$, we have from \cite[Lemma 2.4]{Chen2011normal} that
\begin{equation}
\max\set{\norm{\bts(x)}_\infty, \norm{\bts'(x)}_\infty, \norm{\bts''(x)}_\infty} \le 2\nu B_p.\label{eq:phi_deri_bd}
\end{equation}

In light of (\ref{eq:stein_identity}) and \eref{CLT_1Da}, showing \eref{CLT_1D} boils down to bounding $\left|\E\bts'\left(\frac{\va\tran \wvv}{\nu\sqrt{p}}\right)-\E\frac{\va\tran \wvv}{\nu\sqrt{p}}\bts\left(\frac{\va\tran \wvv}{\nu\sqrt{p}}\right)\right|$. To proceed, we define for every $(i, j)$,
\begin{equation}\label{eq:rhoij}
\rho_{ij}\bydef\frac{\fvec_{i}\tran\fvec_{j}}{\|\fvec_{i}\|^{2}}
\end{equation}
and
\[
\ajmi\bydef\kernel(\cvec\tran \fvec_j - \rho_{ij} \cvec\tran \fvec_i) = \kernel\left(\cvec\tran\left(\mI-\mP_i\right)\fvec_{j}\right),
\]
where $\mP_i = \frac{\fvec_{i}\fvec_{i}\tran}{\|\fvec_{i}\|^{2}}$ denotes the orthogonal projection onto the 1-D space spanned by $\fvec_i$. It is easy to
check that $a_{i}=\kernel(\cvec\tran \fvec_i)$ is independent of $\ajmi$ for all $j\neq i$. It follows that
\begin{equation}\label{eq:ai_aij}
\EE a_i \bts\Big(\tfrac{1}{\nu\sqrt{p}}\sum_{j \neq i} \ajmi\wv_j\Big) = \EE a_i \,\EE \bts\Big(\tfrac{1}{\nu\sqrt{p}}\sum_{j \neq i} \ajmi\wv_j\Big) = 0,
\end{equation}
where the last equality uses the assumption that $\E a_i = 0$ due to $\sigma(x)$ being an odd function. Applying \eref{ai_aij} and after some manipulations, we can verify the following decomposition:
\begin{equation}\label{eq:stein_identity_decomp}
\begin{aligned}
 &\E\Big[\frac{\va\tran \wvv}{\nu\sqrt{p}}\bts\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big)\Big]-\E\bts'\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big) \\
=&  \underbrace{\E\Big[\Big(\frac{1}{\nu\sqrt{p}}\sum_{i=1}^{p}\wv_{i}a_{i}\delta_{i}-1\Big)\bts'\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big)\Big]}_{\text{(a)}} + \\
 & \underbrace{\E\Big\{ \sum_{i=1}^{p}\frac{\wv_{i}a_{i}}{\nu\sqrt{p}}\Big[\bts\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big)-\bts\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}-\delta_{i}\Big)-\bts'\Big(\frac{\va\tran \wvv}{\nu\sqrt{p}}\Big)\delta_{i}\Big]\Big\} }_{\text{(b)}},
\end{aligned}
\end{equation}
where
\begin{equation}
\delta_{i}=\frac{\va\tran \wvv}{\nu\sqrt{p}}-\frac{\sum_{j\neq i}\ajmi \wv_{j}}{\nu\sqrt{p}}.\label{eq:delta_i_def}
\end{equation}
\textcolor[rgb]{0.00,0.00,0.00}{By Stein's identity, when  $\frac{\va\tran \wvv}{\nu\sqrt{p}}$ follows the standard Gaussian distribution, the left-hand side of \eqref{eq:stein_identity_decomp} exactly equals to zero. Intuitively, this quantity should be approximately equal to zero when $\frac{\va\tran \wvv}{\nu\sqrt{p}}$ is approximately standard Gaussian. This is what we are going to prove next.}
In what follows, we derive bounds for the two parts on the right-hand side of (\ref{eq:stein_identity_decomp}), separately.

We start with part (a). To simplify the notation, we let $\chi = \frac{1}{\nu\sqrt{p}}\sum_{i=1}^{p}\wv_ia_{i}\delta_{i}$. Applying the bound on $\left\Vert \bts'(x)\right\Vert _{\infty}$ in \eref{phi_deri_bd} gives us
\begin{align}
\abs{\text{part (a)}} &\le (2\nu B_p) \E\abs{\chi - 1}\nonumber\\
&\le (2\nu B_p) (\E\abs{\chi- \E\chi} + \abs{\E \chi -1})\nonumber\\
&\le (2\nu B_p) (\sqrt{\text{var}(\chi)} +\abs{\E \chi -1}),\label{eq:parta}
\end{align}
where the last step is due to H\"{o}lder's inequality. It is now clear what to do: to show $\text{part (a)} \to 0$, we just need to verify that $\E \chi \to 1$ and $\text{var}(\chi) \to 0$.

Calculating $\E \chi$ is easy. Applying the independence property \eref{ai_aij}, we have
\[
\E \chi = \frac{1}{\nu^2 p} \E \Big[\sum_{i\le p} \wv_i a_i (\va\tran \wvv)\Big] = \frac{1}{\nu^2 p} \wvv\tran \mSig_a \wvv,
\]
where $\mSig_a = \EE \va \va\tran$. One can show that $\mSig_a \approx \mSig_b$, where the latter is defined in \eref{nu}. Specifically, Lemma~\ref{lem:sigma_ab} in Appendix~\ref{appendix:covariance} gives us
\[
\begin{aligned}
    \norm{\mSig_a - \mSig_b} \le& \frac{(1 + \BPf + \norm{\mF}^4)  \polylog p}{\sqrt{p}} \\
    \le& \frac{(1 + \BPf)  \polylog p}{\sqrt{p}},
\end{aligned}
\]
with the second inequality due to \eref{fnorm}. Recall the definition of $\nu$ in \eref{nu}. We then have
\begin{align}
\abs{\E \chi - 1} &= \frac{\abs{\wvv\tran (\mSig_a - \mSig_b) \wvv}}{\nu^2 p} \le \frac{(1 + \BPf ) \polylog p}{\sqrt{p}} \Big(\frac{\norm{\wvv}^2}{\nu^2 p}\Big)\nonumber\\
&\le \frac{(1 + \BPf ) \norm{\wvv}_\infty \norm{\wvv} \polylog p}{\nu^2 p},\label{eq:Echi}
\end{align}
where in the last step we use a simple inequality ($\norm{\wvv}^2 \le \norm{\wvv}_\infty \norm{\wvv} \sqrt{p}$) to bring the final bound to a convenient form.

Next, we consider the variance term in \eref{parta}. Introducing the shorthand notation $u_k = \cvec\tran \fvec_k, 1 \le k \le p$, we rewrite $\delta_i$ in \eref{delta_i_def} as
\begin{align}
\delta_i =& \frac{\wv_i \kernel(u_i)}{\nu \sqrt{p}}  + \frac{1}{\nu \sqrt{p}} \sum_{j \neq i} \wv_j [\kernel(u_j) - \kernel(u_j - \rho_{ij} u_i)]
\nonumber\\
=& \frac{\wv_i \kernel(u_i)}{\nu \sqrt{p}} + \frac{1}{\nu \sqrt{p}} \sum_{j \neq i} \wv_j [\kernel'(u_j)u_i \rho_{ij} - \tfrac{1}{2}\kernel''(u_j)(u_i\rho_{ij})^2 \nonumber\\
&+ \tfrac{1}{6}\kernel'''(\theta_{ij})(u_i\rho_{ij})^3 )],\label{eq:delta_series}
\end{align}
where to reach the second equality we have used Taylor's expansion, with $\theta_{ij}$ denoting a point between $u_j - \rho_{ij} u_i$ and $u_j$. Substituting \eref{delta_series} into the expression for $\chi$ leads to
\begin{equation}\label{eq:X_decomp}
\begin{aligned}
\chi &= \Gamma + \Delta,
\end{aligned}
\end{equation}
where
\begin{equation}
\begin{aligned}
    \Gamma =& \frac{1}{\nu^{2}p}\sum_{i=1}^{p}\left[\wv_i \kernel(u_i)\right]^{2}+\frac{1}{\nu^{2}p}\sum_{i \neq j}\wv_i \wv_j \kernel(u_{i})\big[\kernel'(u_{j})u_{i}\rho_{ij} \\
    &-\frac{1}{2}\kernel''(u_{j})\left(u_{i}\rho_{ij}\right)^{2}\big]
\end{aligned}    
\end{equation}
and
\begin{equation}
    \Delta = \frac{1}{6\nu^{2}p}\sum_{i\neq j}\wv_i \wv_j \kernel(u_{i})\kernel'''(\theta_{ij})\left(u_{i}\rho_{ij}\right)^{3}.
\end{equation}

This then allows us to write
\begin{equation}\label{eq:chi_gamma_delta}
\begin{aligned}
    \sqrt{\text{var}(\chi)} &= \sqrt{\text{var}(\Gamma + \Delta)} \le \sqrt{2 \text{var}(\Gamma) + 2 \E [\Delta^2]} \\
    &\le \sqrt{2 \text{var}(\Gamma)} + \sqrt{2 \E[\Delta^2]}.
\end{aligned}
\end{equation}

The term involving $\Delta$ on the right-hand side of \eref{chi_gamma_delta} is easy to bound, even deterministically. Using our assumptions about the function $\sigma_p(x)$ stated in the lemma, namely it has a compact support and bounded third derivatives, we have $\abs{\kernel(u_i) u_i^3} \le \polylog p$ and $\abs{\kernel'''(\theta_{ij})} \le \polylog p$. In addition, since the feature vectors satisfy \eref{BP}, we can verify from the definition \eref{rhoij} that $\max_{i \neq j} \abs{\rho_{ij}} \le \frac{c \BP}{\sqrt{p}}$ for some constant $c$. It follows that
\begin{equation}\label{eq:Delta_bd}
\left|\Delta\right|  \leq\frac{\BPt \polylog p}{\nu^2p^{5/2}}\sum_{i \neq j} \abs{\wv_i \wv_j} \le \frac{\BPt \norm{\wvv}_\infty \norm{\wvv}\polylog p}{{\nu^2}p},\end{equation}
where the second inequality is due to the simple bound that $\sum_{i \neq j} \abs{\wv_i \wv_j} \le p \norm{\wvv}_\infty  \sum_i \abs{\wv_i} \le p^{3/2} \norm{\wvv}_\infty \norm{\wvv}$.

Now we tackle the more challenging task of bounding $\text{var}(\Gamma)$ in \eref{chi_gamma_delta}. We first note that, since $u_i = \cvec\tran \fvec_i$ and $u_j = \cvec\tran \fvec_j$, we can view $\Gamma$ as a differentiable function of $\cvec$, denoted by $\Gamma(\cvec)$, with $\cvec \sim \mathcal{N}(0, \mI_d)$. The Gaussian Poincar\'{e} inequality (see, \eg, \cite[Theorem 3.20]{boucheron2013concentration}) then gives us
\begin{equation}\label{eq:GP}
\text{var}(\Gamma(\cvec)) \le \E \norm{\nabla \Gamma(\cvec)}^2,
\end{equation}
where the gradient $\nabla \Gamma(\cvec)$ can be computed, with some diligence, as
\begin{align}
 &\nabla\Gamma(\cvec) \nonumber\\
 =& \frac{1}{\nu^{2}p}\Big(\sum_{i\le p}\wv_i^{2}q_1(u_i)\fvec_{i} + \sum_{i \neq j}[\wv_i q'_2(u_i)] [\wv_j q_3(u_j)] \rho_{ij}\fvec_i \nonumber \\ &\hspace{6em} + \sum_{i \neq j}[\wv_i q_2(u_i)] [\wv_j q'_3(u_j)] \rho_{ij}\fvec_j \nonumber \\
 &\hspace{6em} +\sum_{i \neq j}[\wv_i q'_4(u_i)] [\wv_j q_5(u_j)] \rho^2_{ij}\fvec_i \nonumber \\
 &\hspace{6em} + \sum_{i \neq j}[\wv_i q_4(u_i)] [\wv_j q'_5(u_j)] \rho^2_{ij}\fvec_j\Big),\label{eq:grad_gamma}
\end{align}
where $q_1(u) = 2 \kernel(u) \kernel'(u)$, $q_2(u) = \kernel(u) u$, $q_3(u) = \kernel'(u)$, $q_4(u) = -\tfrac{1}{2}\kernel(u) u^2$, and $q_5(u) = \kernel''(u)$.
In light of \eref{GP}, we just need to show that $\norm{\nabla\Gamma(\cvec)}$ is properly bounded. We do so by controlling the norm of each term on the right-hand side of \eref{grad_gamma}.

Note that our assumptions about the function $\sigma_p(x)$ implies that $\norm{q_i(u)}_\infty \le \polylog p$ and $\norm{q'_i(u)}_\infty \le \polylog p$ for $1 \le i \le 5$. Moreover, $\norm{\fmtx} \le \polylog p$ by assumption. Thus, the first term on the right-hand side of \eref{grad_gamma} can be bounded as
\begin{equation}\label{eq:grad_t1}
\Big\Vert{\frac{1}{\nu^2 p}\sum_{i\le p}\wv_i^{2}q_1(u_i)\fvec_{i}}\Big\Vert \le \frac{\norm{\wvv}_\infty \norm{\wvv}\polylog p}{\nu^2 p}.
\end{equation}
For the second term, we first rewrite it in the form of a matrix-vector multiplication as
\[
\frac{1}{\nu^{2}p} \sum_{i \neq j}[\wv_i q'_2(u_i)] [\wv_j q_3(u_j)] \rho_{ij}\fvec_i = \frac{1}{\nu^2 p} \fmtx\mD_1 \mM \mD_2 \wvv,
\]
where $\mD_1 = \diag\left\{ \wv_i q'_2(u_{i})\right\}$, $\mM=\diag\left\{ \|\fvec_{i}\|^{-2}\right\} \fmtx\tran\fmtx-\mI$, and $\mD_2 = \diag\left\{q_3(u_{j})\right\}$.  Clearly, $\norm{\mD_1} \le \norm{\wvv}_\infty \polylog p$ and $\norm{\mD_2} \le \polylog p$. We can also verify that
\begin{equation}\label{eq:rho_mtx}
\norm{\mM} \le c (\norm{\mF}^2 + 1) \le \polylog p.
\end{equation}
It follows that
\begin{equation}\label{eq:grad_t2}
\Big\Vert \frac{1}{\nu^2 p} \sum_{i \neq j}[\wv_i q'_2(u_i)] [\wv_j q_3(u_j)] \rho_{ij}\fvec_i \Big \Vert \le \frac{ \norm{\wvv}_\infty \norm{\wvv}\polylog p}{\nu^2 p}.
\end{equation}
Similarly, the fourth term on the right-hand side of \eref{grad_gamma} can be rewritten as $\frac{1}{\nu^2 p} \fmtx\widetilde{\mD}_1 \widetilde{\mM} \widetilde{\mD}_2 \wvv$, where $\widetilde{\mD}_1 = \diag\left\{ \wv_i q'_4(u_{i})\right\}$, $\widetilde{\mD}_2 = \diag\left\{q_5(u_{j})\right\}$, and $\widetilde{\mM} = \mM \circ \mM$, with $\circ$ denoting the Hadamard product of two matrices. The spectral norm of $\widetilde{\mM}$ can be bounded as
\begin{equation}\label{eq:rho2_mtx}
\norm{\widetilde{\mM}} \le \norm{\widetilde{\mM}}_\text{F} = \big[\textstyle\sum_{i \neq j} \rho_{ij}^4\big]^{1/2} \le c\BPs,
\end{equation}
for some constant $c$, where the last inequality is due to \eref{BP}. This then allows us to bound the norm of the fourth term of the gradient expression as
\begin{equation}\label{eq:grad_t3}
\begin{aligned}
    &\Big\Vert \frac{1}{\nu^2 \sqrt{p}} \sum_{i \neq j}[\wv_i q'_4(u_i)] [\wv_j q_5(u_j)] \rho^2_{ij}\fvec_i\Big\Vert \\
    \le& \frac{ \norm{\wvv}_\infty \norm{\wvv}\BPs\polylog p}{\nu^2 p}.
\end{aligned}
\end{equation}
The situations for the third and fifth term on the right-hand side of \eref{grad_gamma} are completely analogous, and thus we avoid the repetitions. With the bounds in \eref{grad_t1}, \eref{grad_t2} and \eref{grad_t3}, we can now apply \eref{GP} to get
\[
\sqrt{\text{var}(\Gamma)} \le \frac{(1+ \BPs) \norm{\wvv}_\infty \norm{\wvv}\polylog p}{\nu^2 p}.
\]
Combining this bound with those in \eref{Delta_bd}, \eref{chi_gamma_delta}, \eref{Echi}, we can retrace our steps back to \eref{parta} and conclude
\begin{equation}\label{eq:parta_bnd}
\abs{\text{part (a)}} \le   \frac{B_p(1 + \BPf )\norm{\wvv}_\infty\polylog p}{\mu_{2, p} \sqrt{p}},
\end{equation}
where the last inequality also uses the fact that $\mSig_b \succeq \mu_{2, p}^2 \mI$ and thus
\begin{equation}\label{eq:nu_bnd}
\nu \ge \mu_{2,p} \norm{\wvv}/\sqrt{p}.
\end{equation}


Now the remaining task is to bound the part (b) in \eref{stein_identity_decomp} before we can complete the proof. Using Taylor's expansion, we have
\[
\left|\text{part (b)}\right|  =\Big|\frac{1}{2\nu\sqrt{p}}\E\sum_{i=1}^{p}\wv_{i}a_{i}{\bts''(\theta_{i})}\delta_{i}^{2}\Big|
\]
where $\theta_i$ is some point between $\frac{\va\tran \wvv}{\nu\sqrt{p}} - \delta_i$ and $\frac{\va\tran \wvv}{\nu\sqrt{p}}$. By assumption, the function $\kernel(x)$ considered in this lemma is supported on $[-\tau_p, \tau_p]$ for some $\tau_p \le \polylog p$. We can then write $a_i = \kernel(u_i) = \kernel(u_i) \charfn_{[-\tau_p, \tau_p]}(u_i)$. This step of introducing an indicator function is not strictly necessary, but it helps to simplify some of our later arguments. We now have
\begin{align}
\left|\text{part (b)}\right| & =\Big|\frac{1}{2\nu\sqrt{p}}\E\sum_{i=1}^{p}\wv_{i}a_{i}{\bts''(\theta_{i})}\delta_{i}^{2}\charfn_{[-\tau_p, \tau_p]}(u_i)\Big|\nonumber \\
 & \leq\frac{B_p \polylog p}{\sqrt{p}}\linf{\wvv}\sum_{i=1}^{p}\E[\delta_{i}^{2}\charfn_{[-\tau_p, \tau_p]}(u_i)],\label{eq:part_b_bd}
\end{align}
where to reach the last inequality we have also used (\ref{eq:phi_deri_bd}) and the boundedness of $a_i = \kernel(u_i)$. Using a similar Taylor's expansion as in \eref{delta_series} but only to the second order, we have
\[
\begin{aligned}
    &\sum_{i=1}^{p}\E[\delta_{i}^{2}\charfn_{[-\tau_p, \tau_p]}(u_i)] \\
    =& \frac{1}{\nu^2 p}\sum_{i=1}^{p}\E\Big[\wv_{i}a_{i}+\sum_{j\neq i}\big(\kernel'(u_{j})\tilde{u}_{i}\rho_{ij}-\frac{1}{2}\kernel''(\theta_{ij})\left(\tilde{u}_{i}\rho_{ij}\right)^{2}\big)\wv_{j}\Big]^{2},
\end{aligned}
\]
where $\tilde{u}_i \bydef u_i \charfn_{[-\tau_p, \tau_p]}(u_i)$. Expanding the right-hand side of this expression then gives us
\begin{align}
&\abs{\text{part (b)}} \nonumber \\
\leq& \frac{B_p \norm{\wvv}_\infty \polylog p}{\nu^2 p^{3/2}}\Big(\norm{\wvv}^2 +\sum_{i=1}^{p}\E\big[\sum_{j\neq i}\kernel'(u_{j})\rho_{ij}\wv_{j}\big]^{2} \nonumber \\
&\hspace{9em}+\sum_{i=1}^{p}\E\big[\sum_{j\neq i}\kernel''(\theta_{ij})\rho^2_{ij}\wv_{j}\big]^{2}\Big)\nonumber\\
&\le \frac{B_p \norm{\wvv}_\infty \polylog p}{\nu^2 p^{3/2}} (\norm{\wvv}^2 + \E \norm{\mM \diag\set{\kernel'(u_j)} \wvv}^2 \nonumber \\
&\hspace{10em}+\E \norm{\widetilde{\mM} \widetilde{\wvv}}^2),
\end{align}
where $\mM, \widetilde{\mM}$ are the matrices considered in \eref{rho_mtx} and \eref{rho2_mtx}, respectively, and $\widetilde{\wvv} = [\abs{\wv_1}, \ldots, \abs{\wv_p}]\tran$. Using the spectral bounds given in \eref{rho_mtx} and \eref{rho2_mtx}, and the inequality \eref{nu_bnd}, we get
\[
\abs{\text{part (b)}} \le \frac{B_p(1 + \BPf) \norm{\wvv}_\infty \polylog p }{\mu_{2,p}^2\sqrt{p}}.
\]
Substituting this inequality and \eref{parta_bnd} into \eref{stein_identity_decomp}, and using the fact that $\mu_{2,p} \le \polylog p$, we are done.
\end{proof}


\subsection{Joint Distributions}
\label{sec:CLT_cond}

Lemma~\ref{lem:CLT_1D} shows that $\frac{\va\tran \wvv}{\sqrt{p}}$ has an asymptotically Gaussian distribution. Using this result, we can easily show that the asymptotic distribution of $\frac{\va\tran \wvv}{\sqrt{p}}$ and $\cvec\tran \sgl$ is jointly Gaussian, via a conditioning technique.

\begin{lem}\label{lem:CLT_2D}
Consider a sequence of activation functions $\set{\kernel_p(x)}$ and two-dimensional test functions $\set{\btest_p(x; s)}$ such that, for every $p$,
\begin{enumerate}
\item $\kernel_p(x)$ is an odd function;
\item $\max\set{\norm{\sigma'_p(x)}_\infty, \norm{\sigma''_p(x)}_\infty, \norm{\sigma'''_p(x)}_\infty} \le \polylog p$;
\item $\kernel_p(x)$ is compactly supported. Specifically, there is some threshold $\tau_p \le \polylog p$ such that $\kernel_p(x) = 0$ for all $\abs{x} \ge \tau_p$;
\item $\btest_p(x; s)$ is differentiable with respect to $x$. Moreover, there is a function $B_p(s)$ such that
\begin{equation}\label{eq:bps_bnd}
\max\set{\norm{\btest_p(x; s)}_\infty, \norm{\btest'_p(x; s)}_\infty} \le B_p(s).
\end{equation}
\end{enumerate}
For any fixed vectors $\wvv \in \R^p$ and $\sgl \in \R^d$ with $\norm{\sgl} = 1$, it holds that
\begin{equation}\label{eq:CLT_2D}
\begin{aligned}
    &\Big|\EE \btest_p\Big(\frac{\va\tran \wvv}{\sqrt{p}}; \cvec\tran \sgl\Big)-\EE \btest_p\Big(\frac{\vb\tran \wvv}{\sqrt{p}}; \cvec\tran \sgl\Big)\Big| \nonumber \\
    &\hspace{6em}\le \frac{[{\E B_p^2(z)}]^{1/2}(1 + \BPf ) \norm{\wvv}_\infty \polylog p }{\mu_{2,p}^2\sqrt{p}}.
\end{aligned}
\end{equation}
Here, $\vz \sim \mathcal{N}(0, 1)$, $\va, \vb$ are defined the same way as in Lemma~\ref{lem:CLT_1D}, and $\fmtx = [\vf_1, \vf_2, \ldots, \vf_p]$ is a collection of feature vectors satisfying \eref{BP} and \eref{fnorm}.
\end{lem}

\begin{proof}
To lighten the notation, we will omit the subscript $p$ in $\sigma_p(x)$ and $\btest_p(x; s)$ in the proof. The key idea in our proof is to rewrite the jointly Gaussian random variables $\cvec\tran \fmtx$ and $\cvec\tran \sgl$ via an equivalent representation through conditioning. It is easy to check that
\[
(\cvec\tran \fmtx, \cvec\tran \sgl) \overset{\text{Law}}{=} (s \sgl\tran \fmtx + \widetilde{\cvec}\tran (\mI - \sgl \sgl\tran) \fmtx, s),
\]
where $s \sim \mathcal{N}(0, 1)$ and $\widetilde{g} \sim \mathcal{N}(0, \mI_d)$ are two independent sets of Gaussian random variables. Let
\begin{equation}\label{eq:rho_f_tilde}
\rho_i \bydef \sgl\tran \fvec_i, \quad \widetilde{\vf}_i \bydef (\mI - \sgl \sgl\tran) \fvec_i, \quad \text{and} \quad \widetilde{u}_i = \widetilde{\cvec}\tran \widetilde{\fvec}_i.
\end{equation}
We can then redefine the entries of $\va$ and $\vb$ as
\begin{equation}\label{eq:ab_c}
a_i = \kernel(s\rho_i  + \widetilde{u}_i) \quad \text{and} \quad b_i = \mu_{1, p} (s\rho_i  + \widetilde{u}_i) + \mu_{2, p} z_i,
\end{equation}
without changing their probability distributions. The reason we do such decomposition is that $\widetilde{\cvec}\tran \widetilde{\fvec}_i$ is independent of $s$. This convenient independence structure allows us to calculate the expectations in \eref{CLT_2D} by first conditioning on $s$.

Applying Taylor's expansion to the expression for $a_i$ in \eref{ab_c}, we get
\begin{align}
a_{i} & =\kernel(\widetilde{u}_i) + \kernel'(\widetilde{u}_i) s \rho_i + \frac{1}{2}\kernel''\left(\theta_{i}\right)\left(s\rho_{i}\right)^{2}\nonumber \\
 & =\kernel(\widetilde{u}_i) + \mu_{1, p} s \rho_i + [\kernel'(\widetilde{u}_i) -\E\kernel'(\widetilde{u}_i)] (s \rho_i) \nonumber \\
 &~~~+ [\E\kernel'(\widetilde{u}_i) -\mu_{1,p}] (s \rho_i)+ \frac{1}{2}\kernel''\left(\theta_{i}\right)\left(s\rho_{i}\right)^{2},\label{eq:ai_sgl}
\end{align}
where $\theta_i$ is some point between $\widetilde{u}_i$ and $\widetilde{u}_i + s \rho_i$. This expansion then leads to
\[
\E\btest\Big(\frac{\va\tran \wvv}{\sqrt{p}}; \cvec\tran \sgl\Big) = \E\btest\Big(\frac{\sum_i \wv_i \kernel(\widetilde{u}_i)}{\sqrt{p}} +  \frac{s \mu_{1, p}\sum_i \wv_i \rho_i}{\sqrt{p}} + \Delta_1 + \Delta_2; s\Big),
\]
where
\begin{align*}
    \Delta_1 =  \frac{s \sum_i \wv_i \rho_i[\kernel'(\widetilde{u}_i) -\E\kernel'(\widetilde{u}_i)]}{\sqrt{p}}
\end{align*}
and
\begin{align*}
    \quad \Delta_2 = \frac{s \sum_i \wv_i \rho_i[\E\kernel'(\widetilde{u}_i) -\mu_{1,p} + \tfrac{1}{2} \kernel''(\theta_i) s\rho_i]}{\sqrt{p}}.
\end{align*}
Using the bounded derivative assumption in \eref{bps_bnd}, we have
\begin{equation}\label{eq:clt_D1D2}
\begin{aligned}
&\abs{\E\btest\Big(\frac{\va\tran \wvv}{\sqrt{p}}; \cvec\tran \sgl\Big) - \E\btest\Big(\frac{\sum_i \wv_i \kernel(\widetilde{u}_i)}{\sqrt{p}} +  \frac{s \mu_{1, p}\sum_i \wv_i \rho_i}{\sqrt{p}}; s\Big)}\\
&\qquad\qquad\qquad \le \E [B_p(s) (\abs{\Delta_1} + \abs{\Delta_2})] \nonumber\\
&\qquad\qquad\qquad \le [{\E B_p^2(s)}]^{1/2} ([\E \Delta_1^2]^{1/2} +[\E \Delta_2^2]^{1/2}).
\end{aligned}
\end{equation}
Next, we show that the terms involving $\Delta_{1}$ and $\Delta_{2}$ in \eref{clt_D1D2} are small.

The quantity $\E \Delta_1^2$ is small due to concentration. To see that, let $\Gamma_1(\widetilde{\cvec}) \bydef \big[\sum_i \wv_i \rho_i\kernel'(\widetilde{\cvec}\tran \widetilde{\fvec}_i)\big]/\sqrt{p}$. Clearly, $\Delta_1 = s [\Gamma_1(\widetilde{\cvec}) - \E \Gamma_1(\widetilde{\cvec})]$. From the independence of $s$ and $\widetilde{\cvec}$,
\begin{equation}\label{eq:clt_D1_GP}
\E \Delta_1^2 = \text{var}(\Gamma_1(\widetilde{\cvec})) \le \E \norm{\nabla \Gamma_1(\widetilde{\cvec})}^2,
\end{equation}
with the last step being the Gaussian Poincar\'{e} inequality. Recall the definition of $\rho_i$ and $\widetilde{\fvec}_i$ in \eref{rho_f_tilde}. One can verify that
\begin{align}
\norm{\nabla  \Gamma_1(\widetilde{\cvec})} &= \norm{(\mI-\sgl \sgl\tran) \fmtx \diag\set{\rho_i \kernel''(\widetilde{u}_i)} \wvv/\sqrt{p}}\nonumber\\
&\le {\BP (\norm{\wvv}/\sqrt{p}) \polylog p  }/{\sqrt{p}}\label{eq:clt_D1_bnd},
\end{align}
where to reach \eref{clt_D1_bnd} we have used the bound $\max_i \abs{\rho_i} \le \BP/\sqrt{p}$ due to \eref{BP}. Substituting \eref{clt_D1_bnd} into \eref{clt_D1_GP} then gives us
\begin{equation}\label{eq:D1_sq_bnd}
[\E {\Delta_1}^2]^{1/2} \le {\BP  (\norm{\wvv}/\sqrt{p}) \polylog p  }/{\sqrt{p}}.
\end{equation}

To bound $\E \Delta_2^2$, we first note that $\E\kernel'(\widetilde{u}_i) \approx \mu_{1,p}$. More precisely, a simple bound \eref{cov_bnd1} in Appendix~\ref{appendix:covariance} yields
\[
\begin{aligned}
\abs{\E\kernel'(\widetilde{u}_i) - \mu_{1,p}} &\le \polylog p \,\absb{\norm{\widetilde{\fvec}_i}^2 - 1}\\
&= \polylog p \abs{\norm{\fvec_i}^2 - 1 - (\sgl\tran \fvec_i)^2}\\
&\le \BP \polylog p / \sqrt{p}.
\end{aligned}
\]
This then gives us  
$$
\abs{\Delta_2} \le (s^2+\abs{s}) \BPs (\sum_i \abs{\wv_i} / p) \polylog p / \sqrt{p},
$$ and thus
\begin{equation}\label{eq:D2_sq_bnd}
[\E {\Delta_2}^2]^{1/2} \le \BPs (\norm{\wvv}/\sqrt{p}) \polylog p / \sqrt{p}.
\end{equation}
In light of \eref{D1_sq_bnd} and \eref{D2_sq_bnd}, the left-hand side of \eref{clt_D1D2} is well under control.

Using the equivalent representation for $\vb$ in \eref{ab_c}, we have
\[
\EE\btest\Big(\frac{\vb\tran \wvv}{\sqrt{p}}; \cvec\tran \sgl\Big) = \EE{\btest}_\text{shift}\Big(\frac{\sum_i \wv_i (\mu_{1,p} \widetilde{u}_i + \mu_{2, p}z_i)}{\sqrt{p}}; s\Big),
\]
where $\btest_\text{shift}(x; s) \bydef \btest(x + \frac{s \mu_{1, p}\sum_i \wv_i \rho_i}{\sqrt{p}}; s)$ is simply a shifted version of $\btest(x; s)$.
Combining this with \eref{clt_D1D2}, \eref{D1_sq_bnd} and \eref{D2_sq_bnd}, we can now bound the left-hand side (LHS) of \eref{CLT_2D} as
\begin{align}
&\text{LHS of } \eref{CLT_2D} \nonumber \\
\le& \Big|\EE \btest_\text{shift}\Big(\frac{\sum_i \wv_i \widetilde{a}_i}{\sqrt{p}}; s\Big)-\EE \btest_\text{shift}\Big(\frac{\sum_i \wv_i \widetilde{b}_i}{\sqrt{p}}; s\Big)\Big| + \Delta_3\nonumber\\
\le& \E \Big|\EE\big[\btest_\text{shift}(\textstyle\scp\sum_i \wv_i \widetilde{a}_i; s) \mid s\big] \nonumber \\
&\hspace{8em}-\EE\big[\btest_\text{shift}(\scp\sum_i \wv_i \widetilde{b}_i; s) \mid s\big]\Big| + \Delta_3,\label{eq:CLT_2D_cond}
\end{align}
where $\widetilde{a}_i = \kernel(\widetilde{\cvec}\tran \widetilde{\fvec}_i)$, $\widetilde{b}_i = \mu_{1, p} \widetilde{\cvec}\tran \widetilde{\fvec}_i + \mu_{2, p} z_i$, $\E[\cdot \vert s]$ denotes conditional expectation given $s$, and the ``remainder'' term is
\begin{align}
\Delta_3 &=  [{\E B_p^2(s)}]^{1/2}(\BPs + 1) (\norm{\wvv}/\sqrt{p}) \polylog p / \sqrt{p}\nonumber\\
&\le [{\E B_p^2(s)}]^{1/2}(\BPs + 1) \norm{\wvv}_\infty \polylog p / \sqrt{p}\label{eq:remainder}
\end{align}
Note that, for any fixed $s$, we can use Lemma~\ref{lem:CLT_1D} to control the conditional expectation in the first term on the right-hand side of \eref{CLT_2D_cond}. Indeed, with $s$ fixed, $\btest_\text{shift}(x; s)$ can be viewed as a one-dimensional test function and it satisfies all the assumptions stated in Lemma~\ref{lem:CLT_1D}. The only thing that is different here is that we are now using $\{\widetilde{\fvec}_i\}$ as the feature vectors. Thus, to apply Lemma~\ref{lem:CLT_1D}, we need to check that this modified set of feature vectors still satisfy the condition in \eref{BP}. But this is easy to do. Recall that  $\widetilde{\fvec}_i = (\mI - \sgl \sgl\tran) \vf_i$, with $\{\fvec_i\}$ satisfying \eref{BP} for some $\BP = \mathcal{O}(p^{1/8})$. Thus, for all $i, j$,
\[
\begin{aligned}
    \abs{\widetilde{\fvec}_i\tran \widetilde{\fvec}_j-\delta_{ij}} =& \abs{{\fvec_i\tran (\mI - \sgl \sgl\tran) \fvec_j}-\delta_{ij}} \\
    \le& \abs{\fvec_i\tran \fvec_j-\delta_{ij}} + \abs{\sgl\tran \fvec_i} \abs{\sgl\tran \fvec_j} \\
    \le& \frac{\BP}{\sqrt{p}} + \frac{\BPs}{p} \le \frac{c\BP}{\sqrt{p}}
\end{aligned}
\]
for some positive constant $c$. Finally, by substituting the bounds \eref{CLT_1D} [with $B_p$ there replaced by $B_p(s)$] and \eref{remainder} into \eref{CLT_2D_cond}, we reach the target inequality in \eref{CLT_2D}.
\end{proof}


\subsection{Proof of Theorem~\ref{thm:CLT_general}}
\label{sec:CLT_general}

To go from Lemma~\ref{lem:CLT_2D} to Theorem~\ref{thm:CLT_general}, we just need to remove the following two restrictions in the assumptions of Lemma~\ref{lem:CLT_2D}: (1) $\kernel(x)$ is compactly supported on $[-\tau_p, \tau_p]$ for some $\tau_p = \polylog p$; and (2) $\btest(x; s)$ and its derivatives are bounded [see \eref{bps_bnd}]. The main ingredient of our proof is to show, via a standard truncation technique, that the central limit theorem characterization still holds even if we relax these two assumptions.

Let $\btest(x; s)$ be a test function satisfying \eref{btest_condition}. We can construct a smoothly truncated version of this function via
\[
\widehat{\btest}_p(x; s) \bydef \btest(x; s) \strunc_{T_p, 1}(x),
\]
where $\strunc_{T_p, 1}(x)$ is the smooth window function defined in \eref{smooth_ind} in Appendix~\ref{appendix:truncation} and
\begin{equation}\label{eq:Tp}
T_p = (\norm{\fmtx} + 1) (\norm{\wvv}/\sqrt{p}) \sqrt{C_T\log p}
\end{equation}
for some positive constant $C_T$. The threshold $T_p$ in \eref{Tp} is chosen strategically. 
With this choice, we can show
\begin{equation}\label{eq:trunc_test_a_bnd}
\begin{aligned}
    &\E \big|\btest\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)- \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)\big| \\
    \le& [\E B_p^4(z)]^{1/4}(1 + (\norm{\wvv}/\sqrt{p})^{K})\polylog p/\sqrt{p}.
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:trunc_test_b_bnd}
\begin{aligned}
    &\E \big|\btest\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)- \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)\big| \\
    \le& [\E B_p^4(z)]^{1/4}(1 + (\norm{\wvv}/\sqrt{p})^{K})\polylog p/\sqrt{p}.
\end{aligned}
\end{equation}
The detailed proof of \eref{trunc_test_a_bnd} and \eref{trunc_test_b_bnd} are provided in Appendix \ref{subsec:theorem2proof_auxiliary}
 Together, \eref{trunc_test_a_bnd} and \eref{trunc_test_b_bnd} show that replacing the original test function $\btest(x; s)$ with its smoothly truncated approximation $\widehat{\btest}_p(x; s)$ only incurs a small price of $\mathcal{O}(\polylog p/\sqrt{p})$.

Next, we consider the activation function $\kernel(x)$. Using the smooth window function in \eref{smooth_ind} again, we can build a truncated approximation
\begin{equation}\label{eq:kernel_trunc}
\widehat{\kernel}_p(x) \bydef \kernel(x) \strunc_{\tau_p, 1}(x), \quad \text{where }\tau_p = \sqrt{2C_\tau \log p}
\end{equation}
for some positive constant $C_\tau$. It is easy to verify that $\widehat{\kernel}_p(x)$ satisfies all the assumptions stated in Lemma~\ref{lem:CLT_2D} concerning the activation functions. With this truncated activation function, define
\begin{equation}\label{eq:abh_vec}
\widehat{\va} \bydef \widehat{\kernel}_p(\cvec\tran \fmtx) \quad \text{and} \quad \widehat{\vb} \bydef \mu_{1, p} \cvec\tran \fmtx + \mu_{2, p} \vz
\end{equation}
as the counterparts of $\va$ and $\vb$ in \eref{ab_vec}. Here, $\mu_{1, p}, \mu_{2, p}$ are the constants defined in \eref{mu_12p}.
Our goal is to show that $\scp \va\tran \wvv \approx \scp \widehat{\va}\tran \wvv$ and $\scp \vb\tran \wvv \approx \scp \widehat{\vb}\tran \wvv$. 
Specifically, we can get (details are relegated to Appendix \ref{subsec:theorem2proof_auxiliary})
\begin{align}
&\E \big|\widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)- \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\widehat{\va}\tran \wvv; \cvec\tran \sgl\big)\big| \nonumber\\ 
\le&  [\E B_p^4(z)]^{1/4}[1 + (\scp\norm{\wvv})^{2K+1}]  {\polylog p}/{\sqrt{p}}.\label{eq:trunc_kernel_a}
\end{align}
and
\begin{align}
&\E \big|\widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)- \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\widehat{\vb}\tran \wvv; \cvec\tran \sgl\big)\big| \nonumber \\
\le& [\E B_p^4(z)]^{1/4}[1 + (\scp\norm{\wvv})^{2K+1}]\frac{\polylog p}{\sqrt{p}}.\label{eq:trunc_kernel_b}
\end{align}
Given the inequalities in \eref{trunc_test_a_bnd}, \eref{trunc_test_b_bnd}, \eref{trunc_kernel_a} and \eref{trunc_kernel_b}, we have
\[
\begin{aligned}
&\Big|\E \btest\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)-\E \btest\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)\Big| \nonumber\\ 
\le& [\E B_p^4(z)]^{1/4}[1 + (\scp\norm{\wvv})^{2K+1}]\frac{\polylog p}{\sqrt{p}}\\
&\qquad + \Big|\E \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\widehat{\va}\tran \wvv; \cvec\tran \sgl\big)-\E \widehat{\btest}_p\big(\tfrac{1}{\sqrt{p}}\widehat{\vb}\tran \wvv; \cvec\tran \sgl\big)\Big|.
\end{aligned}
\]
We can use Lemma~\ref{lem:CLT_2D} to bound the second term on the right-hand side, since its test function $\widehat{\btest}_p(x; s)$ and the activation function $\widehat{\kernel}_p(x)$ satisfy the assumptions stated in that lemma. Using \eref{CLT_2D} and the property that $\abs{\mu_2 - \mu_{2,p}} \le \polylog p / \sqrt{p}$, we reach the main result \eref{CLT_general} of the theorem.

\subsection{Extension to Piecewise Smooth Test Functions}
\label{sec:CLT_disc}

In what follows, we generalize Theorem~\ref{thm:CLT_general} to test functions that are only piecewise differentiable. This auxiliary result will be needed in our proof of Proposition~\ref{prop:gen} for the case where the ``output function'' $\fout(y)$ in the generalization error \eref{gen_err} lacks smoothness [\eg, $\fout(y) = \sign(y)]$.

\begin{prop}\label{prop:CLT_piecewise}
Consider the same assumptions of Theorem~\ref{thm:CLT_general} with ``$\btest_p(x; s)$ is differentiable with respect to $x$'' replaced by ``$\btest_p(x; s)$ differentiable with respect to $x$ except at a finite number of points $\set{x_1, x_2, \ldots, x_L}$''. Additionally, we also assume that
\begin{enumerate}
\item The upper bound $\BP \le \polylog p$ in \eref{BP}.

\item $\norm{\wvv}_\infty \le \polylog p$.

\item Let $\nu^2 = \wvv\tran \mSig \wvv / p$, where $\mSig$ is the covariance matrix in \eref{Sig}. Then $\nu^2 \ge c > 0$ for some constant $c$.
\end{enumerate}
It then holds that
\begin{equation}\label{eq:CLT_piecewise}
\begin{aligned}
    &\Big|\E \btest_p\big(\tfrac{1}{\sqrt{p}}\va\tran \wvv; \cvec\tran \sgl\big)-\E \btest_p\big(\tfrac{1}{\sqrt{p}}\vb\tran \wvv; \cvec\tran \sgl\big)\Big| \\
    \le& \frac{[\E B^4_p(z)]^{1/4}\polylog p}{p^{1/8}},
\end{aligned}
\end{equation}
where $z\sim\mathcal{N}(0,1)$.
\end{prop}
\begin{rem}
It is possible to improve the convergence rate on the right-hand side of \eref{CLT_piecewise} from $\mathcal{O}(p^{-1/8} \polylog p)$ to $\mathcal{O}(p^{-1/4} \polylog p)$, by requiring higher moments of $B_p(z)$ to be bounded. We do not pursue this optimization as the current form is sufficient for our proof of Proposition~\ref{prop:gen}.
\end{rem}
\begin{proof}
See Appendix \ref{subsec:Proposition3proof}
\end{proof}



==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/command.tex <==
\global\long\def\vct#1{\boldsymbol{#1}}%
\global\long\def\mat#1{\boldsymbol{#1}}%
\global\long\def\opvec{\text{vec}}%
\global\long\def\optr{\mbox{tr}}%
\global\long\def\opmat{\mbox{mat}}%
\global\long\def\opdiag{\mbox{diag}}%

\global\long\def\t#1{\widetilde{#1}}%
\global\long\def\h#1{\widehat{#1}}%
\global\long\def\abs#1{\left\lvert #1\right\rvert }%
\global\long\def\absb#1{\big\lvert #1\big\rvert }%
\global\long\def\norm#1{\lVert#1\rVert}%

\global\long\def\inprod#1{\langle#1\rangle}%
\global\long\def\set#1{\left\{  #1\right\}  }%
\global\long\def\bydef{\overset{\text{def}}{=}}%
\global\long\def\teq#1{\overset{#1}{=}}%
\global\long\def\tleq#1{\overset{#1}{\leq}}%
\global\long\def\tgeq#1{\overset{#1}{\geq}}%
\global\long\def\tapprox#1{\overset{#1}{\approx}}%

\global\long\def\EE{\mathbb{E}\,}%
\global\long\def\EEk{\mathbb{E}_{k}\,}%

\global\long\def\R{\mathbb{R}}%
\global\long\def\E{\mathbb{E}}%
\global\long\def\P{\mathbb{P}}%
\global\long\def\Q{\mathbb{Q}}%
\global\long\def\I{\mathbb{I}}%

\global\long\def\va{\boldsymbol{a}}%
\global\long\def\vb{\boldsymbol{b}}%
\global\long\def\vc{\boldsymbol{c}}%
\global\long\def\vd{\boldsymbol{d}}%
\global\long\def\ve{\boldsymbol{e}}%
\global\long\def\vf{\boldsymbol{f}}%
\global\long\def\vg{\boldsymbol{g}}%

\global\long\def\vh{\boldsymbol{h}}%
\global\long\def\vi{\boldsymbol{i}}%
\global\long\def\vj{\boldsymbol{j}}%
\global\long\def\vk{\boldsymbol{k}}%
\global\long\def\vl{\boldsymbol{l}}%

\global\long\def\vm{\boldsymbol{m}}%
\global\long\def\vn{\boldsymbol{n}}%
\global\long\def\vo{\boldsymbol{o}}%
\global\long\def\vp{\boldsymbol{p}}%
\global\long\def\vq{\boldsymbol{q}}%
\global\long\def\vr{\boldsymbol{r}}%

\global\long\def\vs{\boldsymbol{s}}%
\global\long\def\vt{\boldsymbol{t}}%
\global\long\def\vu{\boldsymbol{u}}%
\global\long\def\vv{\boldsymbol{v}}%
\global\long\def\vw{\boldsymbol{w}}%
\global\long\def\vx{\boldsymbol{x}}%
\global\long\def\vy{\boldsymbol{y}}%
\global\long\def\vz{\boldsymbol{z}}%

\global\long\def\vtheta{\boldsymbol{\theta}}%
\global\long\def\vxi{\boldsymbol{\xi}}%
\global\long\def\vdelta{\boldsymbol{\delta}}%
\global\long\def\veta{\vct{\eta}}%
\global\long\def\vlambda{\boldsymbol{\lambda}}%
\global\long\def\vbeta{\boldsymbol{\beta}}%
\global\long\def\vmu{\boldsymbol{\mu}}%
\global\long\def\vnu{\boldsymbol{\nu}}%
\global\long\def\vsigma{\boldsymbol{\sigma}}%
\global\long\def\vphi{\boldsymbol{\phi}}%
\global\long\def\vrho{\boldsymbol{\rho}}%
\global\long\def\vone{\boldsymbol{1}}%

\global\long\def\mA{\boldsymbol{A}}%
\global\long\def\mB{\boldsymbol{B}}%
\global\long\def\mC{\boldsymbol{C}}%
\global\long\def\mD{\boldsymbol{D}}%
\global\long\def\mE{\boldsymbol{E}}%
\global\long\def\mF{\boldsymbol{F}}%
\global\long\def\mG{\boldsymbol{G}}%

\global\long\def\mH{\boldsymbol{H}}%
\global\long\def\mI{\boldsymbol{I}}%
\global\long\def\mJ{\boldsymbol{J}}%
\global\long\def\mK{\boldsymbol{K}}%
\global\long\def\mL{\boldsymbol{L}}%
\global\long\def\mM{\boldsymbol{M}}%
\global\long\def\mN{\boldsymbol{N}}%

\global\long\def\mO{\boldsymbol{O}}%
\global\long\def\mP{\boldsymbol{P}}%
\global\long\def\mQ{\boldsymbol{Q}}%
\global\long\def\mR{\boldsymbol{R}}%
\global\long\def\mS{\boldsymbol{S}}%
\global\long\def\mT{\boldsymbol{T}}%
\global\long\def\mU{\boldsymbol{U}}%

\global\long\def\mV{\boldsymbol{V}}%
\global\long\def\mW{\boldsymbol{W}}%
\global\long\def\mX{\boldsymbol{X}}%
\global\long\def\mY{\boldsymbol{Y}}%
\global\long\def\mZ{\boldsymbol{Z}}%

\global\long\def\mLa{\boldsymbol{\Lambda}}%
\global\long\def\mOm{\boldsymbol{\Omega}}%
\global\long\def\mPhi{\boldsymbol{\Phi}}%
\global\long\def\mSig{\boldsymbol{\Sigma}}%

\global\long\def\mzero{\boldsymbol{0}}%

\global\long\def\calS{\mathcal{S}}%
\global\long\def\calN{\mathcal{N}}%
\global\long\def\calL{\mathcal{L}}%
\global\long\def\calD{\mathcal{D}}%
\global\long\def\calV{\mathcal{V}}%
\global\long\def\calW{\mathcal{W}}%
\global\long\def\calO{\mathcal{O}}%
\global\long\def\calM{\mathcal{M}}%
\global\long\def\calR{\mathcal{R}}%
\global\long\def\calB{\mathcal{B}}%

\global\long\def\a{\alpha}%
\global\long\def\b{\beta}%
\global\long\def\m{\mu}%
\global\long\def\n{\nu}%
\global\long\def\g{\gamma}%
\global\long\def\s{\sigma}%
\global\long\def\e{\epsilon}%
\global\long\def\w{\omega}%
\global\long\def\veps{\varepsilon}%

\global\long\def\T{\top}%
\global\long\def\d{\text{d}}%

\global\long\def\nt{\left\lfloor nt\right\rfloor }%
\global\long\def\ns{\left\lfloor ns\right\rfloor }%
\global\long\def\textif{\text{if }}%
\global\long\def\otherwise{\text{otherwise}}%
\global\long\def\st{\text{s.t. }}%

\global\long\def\lmax{\lambda_{\max}}%
\global\long\def\lmin{\lambda_{\min}}%

\global\long\def\tvy{\t{\boldsymbol{y}}}%
\global\long\def\tc{\t c}%
\global\long\def\ttau{\t{\tau}}%
\global\long\def\tf{\t f}%
\global\long\def\th{\t h}%
\global\long\def\tq{\t q}%
\global\long\def\tz{\t z}%

\global\long\def\tva{\t{\boldsymbol{a}}}%
\global\long\def\tvw{\t{\boldsymbol{w}}}%
\global\long\def\tw{\t w}%

\global\long\def\asconv{\overset{a.s.}{\longrightarrow}}%
\global\long\def\pconv{\overset{\mathbb{P}}{\longrightarrow}}%
\global\long\def\iid{\overset{i.i.d.}{\sim}}%

\global\long\def\sgl{\boldsymbol{\xi}}%
\global\long\def\noise{\boldsymbol{w}}%
\global\long\def\sgli{\beta}%
\global\long\def\noisei{w}%
\global\long\def\nlob{\mathcal{T}}%

\global\long\def\snr{\text{SNR }}%
\global\long\def\bs{\backslash}%
\global\long\def\diag{\text{diag}}%

\global\long\def\argmin#1{\underset{#1}{\text{\ensuremath{\arg\min} }}}%
\global\long\def\argmax#1{\underset{#1}{\text{\ensuremath{\arg\max}}}}%

\DeclareMathOperator{\prox}{Prox}%
\global\long\def\moreau{\calM}%

\global\long\def\dmtx{\mA}%
\global\long\def\dvec{\va}%
\global\long\def\cmtx{\mG}%
\global\long\def\cvec{\vg}%
\global\long\def\fmtx{\mF}%
\global\long\def\fvec{\vf}%

\global\long\def\svec{\vu}%

\global\long\def\loss{\ell}%
\global\long\def\regu{h}%
\global\long\def\test{\varphi}%
\global\long\def\objfn{U}%
\global\long\def\kernel{\sigma}%

\global\long\def\wt{\vw^{*}}%
\global\long\def\loowt#1{\vw_{#1}^{*}}%
\global\long\def\qwt{\widetilde{\vw}}%

\global\long\def\wti{w^{*}}%

\global\long\def\pathk{\Phi}%
\global\long\def\qpathk{\Psi}%

\global\long\def\field{\theta}%

\global\long\def\ie{\emph{i.e.}}
\global\long\def\eg{\emph{e.g.}}

\global\long\def\terr{\mathcal{E}_\text{train}}
\global\long\def\gerr{\mathcal{E}_\text{gen}}
\global\long\def\terrA{\mathcal{E}_\text{train}(\mA)}
\global\long\def\terrB{\mathcal{E}_\text{train}(\mB)}
\global\long\def\gerrA{\mathcal{E}_\text{gen}(\mA)}
\global\long\def\gerrB{\mathcal{E}_\text{gen}(\mB)}
\global\long\def\gerrLim{\mathcal{E}_\text{gen}^\ast}



\global\long\def\scp{\tfrac{1}{\sqrt{p}}}
\global\long\def\mol{\zeta}
\global\long\def\btest{\varphi}
\global\long\def\bts{\psi}
\global\long\def\strunc{\Omega}
\global\long\def\wv{\beta}
\global\long\def\wvv{\vbeta}
\global\long\def\cv{\vtheta}

\global\long\def\BP{\kappa_p}
\global\long\def\BPs{\kappa^2_p}
\global\long\def\BPt{\kappa^3_p}
\global\long\def\BPf{\kappa^4_p}

\global\long\def\ajmi{\tilde{a}_{j, \bs i}}

\global\long\def\truncmoreau{\widehat{\calM}}%
\global\long\def\trunckernel{\widehat{\kernel}}%

\global\long\def\ptau{P\left(\tau\right)}%
\global\long\def\ltwo#1{\left\Vert #1\right\Vert _{2}}%
\global\long\def\linf#1{\left\Vert #1\right\Vert _{\infty}}%

\global\long\def\Tr{\text{Tr}}%
\global\long\def\sampratio{\text{\ensuremath{\delta_{p}}}}%

\global\long\def\fteacher{\theta_\text{teach}}
\global\long\def\fout{\theta_\text{out}}
\global\long\def\genvar{\rho}
\global\long\def\gencor{\pi}



\global\long\def\epn{m}%
\global\long\def\didx{t}%
\global\long\def\genfn{h}%

\global\long\def\Ecnd#1{\E_{\bs#1}}%
\global\long\def\Pcnd#1{\P_{\bs#1}}%
\global\long\def\Eone#1{\E_{#1}}%

\global\long\def\rhomtx{\mK}%

\global\long\def\Cov{\text{Cov}}%
\global\long\def\lsbd{L_S}% 

==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/conclusion.tex <==
%!TEX root = get_kernel.tex

\section{Conclusion and Final Remarks}
\label{sec:conclusion}

In this paper, we have proved the asymptotic equivalence of a nonlinear random feature model and a surrogate linear Gaussian models in terms of their training and generalization errors. As a consequence of this universality theorem, the learning performance of high-dimensional random feature models can be precisely characterized by studying their linear Gaussian counterparts, which are much more amenable to theoretical analysis. Our proof, which builds on the classical Lindeberg approach, makes several technical assumptions on the loss function, the nonlinear activation function, and the feature matrix. We close the paper by discussing how some of these assumptions can be further relaxed.

\emph{Non-differentiable loss functions.} In Assumption~\ref{a:loss}, we require the loss function $\loss(x; y)$ to have bounded third partial derivatives with respect to $x$. Many loss functions used in practice are not differentiable everywhere. A notable example is the hinge loss for binary classification, where $\loss(x; y) = \ell_\text{hinge}(yx)$ with $\ell_\text{hinge}(x) = \max(0, 1-x)$. One way to extend our current analysis to such non-differentiable functions is to consider a smoothed approximation via convolution. In the case of the hinge loss, let
\[
\ell_{\text{hinge},\delta}(x) =  \int_{\R} \ell_\text{hinge}(x-z)\mol_\delta(z) dz,
\]
where $\mol_\delta(z)$ is a scaled mollifier defined in \eref{sc_mol}. It is easy to verify that, for every $\delta > 0$, $\ell_{\text{hinge},\delta}(x)$ is convex, $\norm{\ell'''_{\text{hinge},\delta}(x)}_\infty \le C / \delta^3$, and
\begin{equation}\label{eq:hinge_smooth_bnd}
\norm{\ell_\text{hinge}(x) - \ell_{\text{hinge},\delta}(x)}_\infty \le C\delta,
\end{equation}
for some $C > 0$. Recall that $\Phi_{\mA}$ and $\Phi_{\mB}$ denote the training errors [\emph{i.e.},\ the minimum value of the optimization problem in \eref{gen_opt}] of the nonlinear feature model and the linear Gaussian model, respectively. We now use $\Phi_{\mA}^\delta$ and $\Phi_{\mB}^\delta$ to denote the corresponding quantities if we replace the hinge loss in \eref{gen_opt} by its smooth version $\ell_{\text{hinge},\delta}(x)$. It follows from \eref{hinge_smooth_bnd} that $\abs{\tfrac{1}{p}\Phi_{\mA} - \tfrac{1}{p}\Phi_{\mA}^\delta} \le C(n/p)\delta$ and $\abs{\tfrac{1}{p}\Phi_{\mB} - \tfrac{1}{p}\Phi_{\mB}^\delta} \le C(n/p)\delta$. The left-hand side of \eref{test_func} can now be bounded as
\begin{equation}\label{eq:test_hinge_smooth}
\begin{aligned}
    &\abs{\E \test(\tfrac{1}{p}{\Phi_{\mA}}) -  \E \test(\tfrac{1}{p}{\Phi_{\mB}})} \\
    &\quad\le 2C(n/p) \norm{\test'}_\infty \delta + \abs{\E \test(\tfrac{1}{p}{\Phi_{\mA}^\delta}) -  \E \test(\tfrac{1}{p}{\Phi_{\mB}^\delta})}.
\end{aligned}
\end{equation}
Since $\ell_{\text{hinge},\delta}(x)$ satisfies Assumption~\ref{a:loss}, we can apply our current analysis to bound the second term on the right-hand side of \eref{test_hinge_smooth}. We have the freedom in choosing the parameter $\delta$. Clearly, $\delta$ must go to $0$ as $p \to \infty$, but it cannot be too small. This is because $\norm{\ell'''_{\text{hinge},\delta}(x)}_\infty \le C / \delta^3$, and this bound on the third derivative is hidden in our estimates in Lemma~\ref{lem:qwt_wt_deterministic_bd}, Lemma~\ref{lem:optwt_qwt_prob_bd} and Lemma~\ref{lem:wk_qwtk_diff_moments_bd}. By choosing an optimal rate of decay for $\delta$, we can show that the left-hand side of \eref{test_hinge_smooth} tends to $0$ as $p$ grows, albeit with a slower convergence rate than that given in \eref{test_func}. Note that similar smoothing techniques can also be used to extend our analysis to non-differentiable activation functions and regularizers.

\emph{More general activation functions.} As a main limitation of our current work, we have assumed that the activation function $\kernel(x)$ is odd. Under this assumption, the regression vectors $\set{\va_t}$ in \eref{a_vec} and $\set{\vb_t}$ in \eref{b_vec} have zero mean and this simplifies our proof. As shown in \fref{quadratic}, the universality phenomenon holds under more general activation functions, including \emph{e.g.}, $\kernel(x) = \max(x, 0)$. One possible way to extend our work to such cases is the following. Let $\widetilde{\va}_t = \va_t - \mu_0 \vone$ and $\widetilde{\vb}_t = \vb_t - \mu_0 \vone$, where $\mu_0$ is the constant in \eref{mu_constants}. Then $\widetilde{\va}_t$ and $\widetilde{\vb}_t$ have (approximately) zero mean. We also rewrite the optimization problem in \eref{gen_opt} as an equivalent two stage process: $\Phi_{\mA}(\tau_1, \tau_2) = \min_{c \in \R} \Phi_{\mA}(c, \tau_1, \tau_2)$, where
\[
\begin{aligned}
    &\Phi_{\mA}(c, \tau_1, \tau_2) \\
    =& \inf_{\vone\tran \vw / \sqrt{p} = c} \big\{\textstyle\sum_{\didx=1}^{n} \loss(\tfrac{1}{\sqrt{p}}\widetilde{\va}_\didx\tran \vw + \mu_0 c; y_\didx) + \\
    &\qquad\qquad\quad \sum_{j = 1}^p \regu(w_j) + {\tau_1} (\vw\tran \mSig \vw) + \tau_2 (\sqrt{p} \mu_1\sgl\tran \fmtx \vw)\big\}.
\end{aligned}
\]
We can define $\Phi_{\mB}(c, \tau_1, \tau_2)$ in a similar way. Since $\E[\widetilde{\va}_t] \approx \mathbf{0}$ and $\E[\widetilde{\vb}_t] = \mathbf{0}$, it is not difficult to extend our current analysis to show that $\Phi_{\mA}(c, \tau_1, \tau_2)/p \approx \Phi_{\mB}(c, \tau_1, \tau_2) / p$. The remaining challenge is to show that this approximate equivalence holds uniformly over $c$, potentially by exploiting the convexity of the functions $\Phi_{\mA}(c, \tau_1, \tau_2)$ and $\Phi_{\mA}(c, \tau_1, \tau_2)$ with respect to $c$.

\emph{Deterministic feature matrices.} Yet another limitation of our work is that we have only considered cases where the columns of the feature matrix $\fmtx$ are independent Gaussian vectors. In fact, most of our technical results (such as those stated in \sref{Lindeberg}) have been obtained when we condition on a \emph{fixed} $\fmtx$ that satisfies \eref{BP} and \eref{fnorm}. The only place where we use the randomness of $\fmtx$ is in Lemma~\ref{lem:loowt_l_infty_bd} and Proposition~\ref{prop:wt_bnd}, where we show that the $\ell_\infty$-norm of the optimal weight vector $\wt_k$ is bounded by $\polylog p$ with high probability. This bound on the $\ell_\infty$-norm is needed in the central limit theorem stated in Theorem~\ref{thm:CLT_general}. [See, in particular, \eref{CLT_general}.] Thus, an important open problem is to check if $\norm{\wt_k}_\infty \le \polylog p$ with high probability for deterministic feature matrices that satisfy \eref{BP} and \eref{fnorm}. 

==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/introduction.tex <==
%!TEX root = get_kernel.tex
\section{Introduction}

\subsection{Background and Motivation}
Consider a supervised learning problem with a collection of training samples $\set{\cvec_\didx, y_\didx}_{1 \le \didx \le n}$. We seek to learn a relationship between the input $\cvec_\didx \in \R^d$ and the output $y_\didx \in \R$ by fitting the training data on a parametric family of functions in the form of
\[
\big\{Y_{\vw}(\cvec) = \scp \vw\tran \mathcal{T}(\cvec): \vw \in \R^p\big\},
\]
where $\mathcal{T}: \R^d \mapsto \R^p$ is a (possibly nonlinear and stochastic) feature map. Each such function $Y_{\vw}(\cvec)$ is indexed by a weight vector $\vw$, and we choose the optimal $\vw$ by solving an optimization problem
\begin{equation}\label{eq:training}
\wt_{\mR} = \argmin{\vw \in \R^p} \textstyle\sum_{\didx = 1}^{n} \loss(\tfrac{1}{\sqrt{p}}\vr_{\didx}\tran \vw; y_\didx) + \sum_{j=1}^{p} \regu(w_j).
\end{equation}
Here, $\loss(x; y)$ is a loss function, $\regu(x)$ is a regularizer, and $\mR = [\vr_1, \vr_2, \ldots, \vr_n]\tran \in \R^{n \times p}$ denotes the matrix whose rows are the regressors used in \eref{training}, \ie,
\begin{equation}\label{eq:regressor}
\vr_\didx = \mathcal{T}(\cvec_\didx), \qquad 1 \le \didx \le n.
\end{equation}
Examples of the loss function include the squared loss [$\loss(x, y) = \tfrac{1}{2}(x-y)^2$] and the logistic loss [$\loss(x, y) = \log(1+e^{-yx})$]. The latter is often used in binary classification tasks, where the labels $y_\didx \in \set{\pm 1}$.

The supervised learning process described above has two main performance metrics: the \emph{training error}
\begin{equation}\label{eq:training_error}
\terr(\mR) = \frac{1}{p} \big\{\textstyle\sum_{\didx=1}^{n} \loss(\scp \vr_\didx\tran \wt_{\mR}; y_\didx) + \sum_{j=1}^{p}\regu(w^\ast_{\mR,j})\big\},
\end{equation}
which is simply a scaled version of the optimal value of \eref{training}, and the \emph{generalization error}
\begin{equation}\label{eq:gen_err}
\gerr(\mR) = \EE \big(y_\text{new} - {\fout}[\scp(\wt_{\mR})\tran \mathcal{T}(\cvec_\text{new})]\big)^2,
\end{equation}
where $\fout(\cdot)$ is some post-processing function (\eg, the sign function) and the expectation in \eref{gen_err} is taken over a fresh pair of samples $\set{\cvec_\text{new}, y_\text{new}}$ that are independent of the training data. To carry out theoretical analysis of the training and generalization errors, it is necessary to make some further assumptions on how the training samples $\set{\cvec_\didx, y_\didx}$ are generated. A classical model, which is also the one adopted in this work, is the so-called teacher-student framework. Specifically, we assume that $\cvec_\didx \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, \mI_d)$ and
\begin{equation}\label{eq:teacher}
y_\didx = \fteacher(\cvec_\didx\tran \sgl),
\end{equation}
where $\sgl \in \R^d$ is a fixed and unknown \emph{teacher vector}, and $\fteacher(\cdot)$ is an unknown function.

In this paper, we study a particular case of the above setting, known in the literature as the \emph{random feature model} \cite{rahimi2008random}. It corresponds to specializing the general regressors in \eref{regressor} to
\begin{equation}\label{eq:a_vec}
\vr_\didx = \va_\didx \bydef \kernel(\fmtx\tran \cvec_\didx),
\end{equation}
where $\fmtx \in \R^{d \times p}$ is a random feature matrix, and $\kernel: \R \mapsto \R$ is a nonlinear scalar activation function [\eg, $\kernel(x) = \tanh(x)$] applied to individual elements of $\mF\tran \cvec_\didx$. Alternatively, the model in \eref{a_vec} can be viewed as a two-layer neural network, with $\cvec_\didx$ being the input to the network, $\fmtx$ the weight matrix in the first layer, and $\kernel(x)$ the activation function. The optimization in \eref{training} (with $\set{\vr_\didx}$ replaced by $\set{\va_\didx}$) then corresponds to learning $\vw$, the second-layer weights of the network, with the first layer weights $\fmtx$ kept fixed.

The random feature model has received considerable attention in the last few years mainly due to its impressive performance and its connection to overparameterized neural networks \cite{rahimi2008random,daniely2016toward,daniely2017sgd,bach2017equivalence,jacot2018neural,belkin2018understand,liu2020random}.
%For example, it is shown in some cases, the functions produced by neural networks corresponds to regression under certain random feature models .
Some of that attention has been directed towards analyzing the performance of this model in high-dimensional regimes. Developments along this line can be found in \emph{e.g.}, \cite{louart2018random,hastie2019surprises,mei2019generalization,montanari2019generalization,goldt2019modelling,gerace2020generalisation,Goldt2020Gaussian, ghorbani2019linearized,ba2019generalization,dhifallah2020precise}. In \cite{louart2018random,mei2019generalization}, the authors precisely characterized the training and generalization errors associated with a special case of \eref{training}, where the loss function $\loss(x; y) = \tfrac{1}{2}(x-y)^2$ and the regularization function is $\regu(x) = \tfrac{\lambda}{2} x^2$. This setting, known as ridge regression, has a closed-form solution. By studying a corresponding (kernel) random matrix, one can show that $\terr$ and $\gerr$ converge to well-defined deterministic limits as the number of training samples $n$ and the problem dimensions $d, p$ grow to infinity at fixed ratios. However, it is difficult to extend such analysis to more general (non-quadratic) loss and regularization functions for which no closed-form solution exists. In particular, the presence of the nonlinear activation function $\kernel(x)$ in \eref{a_vec} makes the regressors $\set{\va_t}$ in \eref{a_vec} non-Gaussian. This then prevents the direct application of analysis tools such as Gaussian min-max theorems (GMT) \cite{gordon1985some,thrampoulidis2018precise}, Gaussian width \cite{chandrasekaran2012convex}, or statistical dimensions \cite{amelunxen2014living}, as they have all been built for analyzing problems involving Gaussian vectors.

%it difficult to use technical tools such as the Gaussian min-max theorem (GMT) \cite{} or the geometric framework based on Gaussian width \cite{} and statistical dimensions \cite{}.

\subsection{The Gaussian Equivalence Conjecture}
Fortunately, it has been observed by many authors (see, \eg, \cite{hastie2019surprises,mei2019generalization,montanari2019generalization,goldt2019modelling, gerace2020generalisation,Goldt2020Gaussian,dhifallah2020precise,seddik2020random,Dhifallah2021inherent,Loureiro2021capturing}, and also \cite{cheng2013spectrum,pennington2017nonlinear,louart2018random} in the context of random kernel matrices) that the random feature model considered above should be asymptotically equivalent to a Gaussian model, where we set the regressors in \eref{regressor} to
\begin{equation}\label{eq:b_vec}
\vr_\didx = \vb_\didx \bydef \mu_0 \vone + \mu_1 \fmtx\tran \cvec_\didx + \mu_2 \vz_\didx.
\end{equation}
Here, $\vone$ denotes an all-one vector in $\R^p$, $\vz_\didx \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, \mI_p)$ is independent of $\cvec_\didx$, and $\mu_0, \mu_1, \mu_2$ are three constants defined as follows. Let $z$ be a standard Gaussian random variable, then
\begin{equation}\label{eq:mu_constants}
\begin{aligned}
   \mu_0 &= \EE[\kernel(z)], \quad \mu_1 = \EE[z\kernel(z)]\quad \text{and} \\ \quad \mu_2 &= (\EE[\kernel^2(z)] - \mu_0^2 - \mu_1^2)^{1/2}. 
\end{aligned}
\end{equation}
In what follows, we shall refer to the setting where the regressors are $\set{\va_\didx}$ in \eref{a_vec} as the \emph{nonlinear feature model}, and refer to the one using $\set{\vb_\didx}$ in \eref{b_vec} as the \emph{linear Gaussian model}. Let
\begin{equation}\label{eq:mat_AB}
\mA = [\va_1, \va_2, \ldots, \va_n]\tran \quad \text{and} \quad \mB = [\vb_1, \vb_2, \ldots, \vb_n]\tran.
\end{equation}
The optimal weight vectors, the training and the generalization errors of these two formulations can then be written as $\wt_{\mA}, \wt_{\mB}$, $\terrA, \terrB$, and $\gerrA, \gerrB$, respectively.

Roughly speaking, the \emph{Gaussian equivalence conjecture} states that, under certain conditions on the feature matrix $\fmtx$, we have
\begin{equation}\label{eq:asymp_equiv}
\terrA \approx \terrB \quad \text{and} \quad \gerrA \approx \gerrB \quad \text{as } p \to \infty.
\end{equation}

\begin{example}
We illustrate this conjecture with two numerical examples. \fref{quadratic} shows the training and generalization errors of a regression problem, where $\fteacher(x) = \fout(x) = x$ and $\kernel(x) = \max(x, 0)$ is the ReLU function. The feature matrix $\fmtx$ in \eref{a_vec} is chosen to be a random matrix with i.i.d. normal entries drawn from $\mathcal{N}(0,1/d)$. To find the optimal weight vector in \eref{training}, we use a quadratic loss $\loss(x; y) = \tfrac{1}{2}(x-y)^2$ and a ridge regularizer $\regu(x) = \frac{\lambda}{2}x^2$. We can see from the simulation results that, even at a moderate problem size ($d=200$ and $n = 600$), the training and generalization errors under the nonlinear feature model and the corresponding linear Gaussian model are already very close. Moreover, they match the analytical predictions developed for the Gaussian model \cite{dhifallah2020precise}. The same phenomenon can also been observed in \fref{logistic}, where we consider a binary classification problem with $\fteacher(x) = \fout(x) = \sign(x)$ and $\kernel(x) = \tanh(x)$. The loss function here is the logistic loss $\loss(x, y) = \log(1+e^{-yx})$, and the regularizer is $\regu(x) = \frac{\lambda}{2}x^2$.
\end{example}

\begin{figure}[t]
\centering
\subfigure[linear regression]{\label{fig:quadratic}
\includegraphics[scale=0.45]{fig/quadratic}}
\hspace{6ex}
\subfigure[binary classification]{\label{fig:logistic}
\includegraphics[scale=0.45]{fig/logistic}}
\caption{Numerical simulations to demonstrate the asymptotic Gaussian equivalence stated in \eref{asymp_equiv}. (a) A regression problem, where the activation function $\kernel(x) = \max(x, 0)$, the loss function $\ell(x; y)$ is the quadratic function, and $\fteacher(x) = \fout(x) = x$. (b) A binary classification problem, where $\kernel(x) = \tanh(x)$, $\ell(x; y)$ is the logistic loss, and $\fteacher(x) = \fout(x) = \sign(x)$. In both cases, we set $d=200$ and $n=600$, and vary the values of $p$. The simulation results are averaged over 100 independent trials, and the theoretical curves are the analytical predictions \cite{dhifallah2020precise} developed for the Gaussian model.}\label{fig:universality_sim}
\end{figure}

That the nonlinear feature model and the linear Gaussian model can be asymptotically equivalent has a simple intuitive explanation. Under certain conditions on the random feature matrix $\fmtx$, one can show that the random vectors $\va_\didx$ in \eref{a_vec} and $\vb_\didx$ in \eref{b_vec} have asymptotically matching first and second moments. (See Appendix~\ref{appendix:covariance} for details.) Thus, the asymptotic equivalence in \eref{asymp_equiv} points to the emergence of a \emph{universality phenomenon} that is inherent in many large random systems: The macroscopic behaviors of such systems only depend on a few key parameters (the first two moments of $\va_\didx$ and $\vb_\didx$ in our case), whereas the microscopic structures of the systems (\emph{i.e.}, the exact probability distributions of $\va_\didx$ and $\vb_\didx$) are irrelevant.

Notice that the surrogate Gaussian formulation is much more amenable to theoretical analysis, as it only involves Gaussian vectors $\set{\vb_\didx}$. Indeed, based on the Gaussian equivalence conjecture, the authors of \cite{montanari2019generalization} provided a precise asymptotic characterization of maximum-margin linear classifiers in the overparameterized regime using Gaussian min-max theorems \cite{gordon1985some,thrampoulidis2018precise}. The performance of the linear Gaussian model under more general settings, where one uses generic convex loss functions and ridge regularization in \eref{training}, was studied in \cite{gerace2020generalisation} by using the non-rigorous replica method \cite{mezard1987spin} from statistical physics. More recently, these replica predictions have been rigorously proved in \cite{dhifallah2020precise}.

\subsection{Main Contributions}

The main contribution of this paper is to prove the aforementioned Gaussian equivalence conjecture. Our results are based on the following technical assumptions.

\newcounter{assumptions}
\begin{enumerate}[label={(A.\arabic*)}]
\item \label{a:Gaussian} The latent input vectors $\cvec_\didx \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, \mI_d)$ in \eref{a_vec} and \eref{b_vec}.

\item \label{a:dimensions} The dimension of the latent input vectors $\cvec_\didx$ (denoted by $d$), the dimension of the regression vectors (denoted by $p$), and the number of training samples (denoted by $n$) tend to infinity at fixed ratios. Specifically, $n / d \to \alpha > 0$ and $p / d \to \eta > 0$ as $d \to \infty$.

\item \label{a:sgl} The unknown teacher vector $\sgl$ in \eref{teacher} is deterministic, with $\norm{\sgl} = 1$.

\item \label{a:loss} The loss function $\loss(x; y)\ge 0$ for all $x, y$, and it is convex with respect to its first variable $x$. The third partial derivative of $\loss(x; y)$ with respect to $x$ exists. Moreover, there exist constants $C>0$ and $K_1 \in\mathbb{Z}^{+}$ such that
\[
\abs{\loss'''(x; \fteacher[s])} \le C(1+|s|^{K_1}), \quad \text{for all }x \in \R,
\]
and
\begin{align*}
    &\max\set{\abs{\loss(0; \fteacher[s])}, \abs{\loss'(0; \fteacher[s])}, \abs{\loss''(0; \fteacher[s])}} \\
    &\le C(1+|s|^{K_1}),
\end{align*}
where $\fteacher(\cdot)$ is the function in \eref{teacher}.
%\[
%\abs{\loss'''(x; y)} \le (\abs{x}^K + 1) B(y),
%\]
%for some positive constant $K$ and function $B(y)$ such that
%\[
%\EE B^4[\varphi(z)] < \infty,
%\]
%where $z \sim \mathcal{N}(0, 1)$ and $\varphi(\cdot)$ is the function in \eref{teacher}.
%Moreover, there exists two positive constants $C_1, C_2$ such that
%\begin{equation}\label{eq:orgin_bnd}
%\P\Big[\frac{1}{n}\sum_{i=1}^n \loss(0; \varphi(s_i)) \ge C_1\Big] \le C_2 e^{-p / C_2},
%\end{equation}
%where $s_1, s_2, \ldots, s_n \overset{\text{i.i.d.}}{\sim} \mathcal{N}(0, 1)$.

\item \label{a:regu} The regularizer $h(\cdot)$ in \eref{training} is strongly convex with parameter $\lambda > 0$. In addition, $h'''(x)$ exists, and it is uniformly bounded over $x \in \R$.

\item \label{a:kernel} The activation function $\kernel(\cdot)$ is an odd function, with bounded first, second, and third derivatives.

\item \label{a:fout} The function $\fout(x)$ in \eref{gen_err} is differentiable except at a finite number of points $\set{x_1, x_2, \ldots, x_L}$. Moreover, there exist constants $C>0$ and $K_2 \in \mathbb{Z}^+$ such that
\[
\max\set{\abs{\fteacher(x)}, \abs{\fout(x)}} \le C(1 + \abs{x}^{K_2}), ~\text{for all }x \in \R
\]
and
\[
\abs{\fout'(x)} \le C(1 + \abs{x}^{K_2}),\quad \text{for } x \not\in \set{x_1, x_2, \ldots, x_L}.
\]

\item \label{a:feature} The columns of the feature matrix $\fmtx = [\vf_1, \vf_2, \ldots, \vf_p]$ are independent Gaussian random vectors: $\vf_i \overset{\text{i.i.d.}}{\sim} \mathcal{N}(\mzero, \tfrac{1}{d}\mI_d)$ for $1 \le i \le p$. Moreover, $\fmtx$ is independent of the latent input variables $\set{\cvec_\didx}$.
\setcounter{assumptions}{\value{enumi}}
\end{enumerate}

\begin{rem}
We can verify that the conditions in Assumption \ref{a:loss} are satisfied by the quadratic loss function, the logistic loss function, and by any $\fteacher(s)$ that grows no faster than some polynomial of $\abs{s}$ as $\abs{s} \to \infty$. Possible ways to generalize our results to non-differentiable loss functions (\emph{e.g.} the hinge loss) will be discussed in \sref{conclusion}. To simplify our analysis, we require in Assumption~\ref{a:kernel} that the activation function $\kernel(x)$ be odd, which then implies that $\mu_0 = 0$ in \eref{mu_constants}. This is merely a limitation of our current results, and the asymptotic equivalence in \eref{asymp_equiv} is expected to hold for more general activation functions [such as the ReLU function as shown in \fref{quadratic}]. Yet another limitation of our work is the Gaussian assumption on the feature vectors in Assumption~\ref{a:feature}. With some extra effort (mostly on generalizing the concentration inequalities in Appendix~\ref{appendix:Concentration_Lipschitz}), our proof can be easily extended to cases where the columns of the feature matrix are independent sub-Gaussian random vectors. However, we expect that the majority of our proof technique should work for \emph{deterministic} feature matrices that satisfy the conditions in \eref{BP} and \eref{fnorm}. We will elaborate on this point in \sref{conclusion} and pinpoint the one technical difficulty that prevents us from working with deterministic matrices.
\end{rem}

To state the results of our main theorem, we first introduce a perturbed version of the optimization problem in \eref{training}:
\begin{equation}\label{eq:gen_opt}
\begin{aligned}
    \Phi_{\mR}(\tau_1, \tau_2) \bydef& \inf_{\vw \in \R^p} \big\{\textstyle\sum_{\didx=1}^{n} \loss(\tfrac{1}{\sqrt{p}}\vr_\didx\tran \vw; y_\didx) + \sum_{j = 1}^p \regu(w_j) \\
    &\hspace{2.5em}+ {\tau_1} (\vw\tran \mSig \vw) + \tau_2 (\sqrt{p} \mu_1\sgl\tran \fmtx \vw)\big\},
\end{aligned}
\end{equation}
where $\tau_1, \tau_2$ are two parameters, $\sgl$ is the teacher vector in \eref{teacher}, and
\begin{equation}\label{eq:Sig}
\mSig \bydef \mu_1^2 \fmtx\tran \fmtx + \mu_2^2 \mI_p.
\end{equation}
Note that $\tfrac{1}{p}\Phi_{\mA}(0, 0)$ and $\tfrac{1}{p}\Phi_{\mB}(0, 0)$ [with the regressor matrix $\mR$ specialized to $\mA$ and $\mB$ in \eref{mat_AB}] are exactly the training errors associated with the feature and Gaussian formulations, respectively. The two extra terms $\tau_1 (\vw\tran \mSig \vw)$ and $\tau_2 (\sqrt{p} \mu_1\sgl\tran \fmtx \vw)$ in \eref{gen_opt} will be needed in our analysis of the generalization error. In particular, we shall consider different values of $\tau_1, \tau_2$ such that
\begin{equation}\label{eq:tau12}
\abs{\tau_1} \le \tau^\ast \bydef \frac{\lambda/4}{\mu_1^2 (1+2\sqrt{\eta})^2 + \mu_2^2} \quad \text{and} \quad \abs{\tau_2} \le 1.
\end{equation}

\begin{rem}\label{rem:convex}
The bound $\tau^\ast$ requires some explanation. At first glance, the possibility that $\tau_1$ can take negative values is worrisome, as $\tau_1 \vw\tran \mSig \vw$ will then be a \emph{concave} function of $\vw$. This concave term, however, will (most likely) not change the convexity of the overall objective function in \eref{gen_opt}. To see this, we recall from Assumption~\ref{a:feature} that $\fmtx\tran \fmtx$ has a Wishart distribution and thus its spectral norm is bounded with high probability. Specifically, it is easy to show (see Appendix~\ref{appendix:matrix}) that
\[
\P(\norm{\fmtx} \ge 1+2\sqrt{\eta}) \le 2 e^{-c p},
\]
where $\eta = p/d$ and $c$ is some positive constant. By Assumption~\ref{a:regu}, the regularizer $h(x)$ is strongly convex with parameter $\lambda > 0$. It follows that, with $\tau_1 \ge -\tau^\ast$, the overall objective function of \eref{gen_opt} is $\frac{\lambda}{2}$-strongly convex with probability at least $1 - 2e^{-cp}$,
\end{rem}


\begin{thm}\label{thm:get}
Suppose Assumptions~\ref{a:Gaussian}--\ref{a:feature} hold. Fix $\tau_1 \in [-\tau^\ast, \tau^\ast]$ and $\tau_2 \in [-1, 1]$. For every $\varepsilon \in (0, 1)$ and every finite constant $c$, we have
\begin{equation}\label{eq:get}
\begin{aligned}
    &\P(\abs{\Phi_{\mA}(\tau_1, \tau_2)/p - c} \ge 2\varepsilon)\\
    \le& \P(\abs{\Phi_{\mB}(\tau_1, \tau_2)/p - c} \ge \varepsilon) 
    + \frac{\polylog p}{\varepsilon \sqrt{p}}
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:get2}
\begin{aligned}
    &\P(\abs{\Phi_{\mB}(\tau_1, \tau_2)/p - c} \ge 2\varepsilon) \\
    \le& \P(\abs{\Phi_{\mA}(\tau_1, \tau_2)/p - c} \ge \varepsilon) + \frac{\polylog p}{\varepsilon \sqrt{p}},
\end{aligned}
\end{equation}
for $p \ge 1/\varepsilon^2$, where $\polylog p$ denotes some function that grows no faster than a polynomial of $\log p$. Consequently,
\begin{equation}\label{eq:get_cip}
\frac{\Phi_{\mA}(\tau_1, \tau_2)}{p} \cip c \quad \text{if and only if} \quad \frac{\Phi_{\mB}(\tau_1, \tau_2)}{p} \cip c,
\end{equation}
where $\cip$ denotes convergence in probability as $p \to \infty$.
\end{thm}

\begin{rem}
We prove this theorem in \sref{get}. A special case, with $\tau_1 = \tau_2 = 0$, implies that the training errors of the nonlinear feature model and its Gaussian surrogate must necessarily have the same asymptotic limit.
\end{rem}

The next result, whose proof can be found in \sref{proof_gen}, establishes the universality for the generalization error, under one additional assumption:
\begin{enumerate}[label={(A.\arabic*)}]
\setcounter{enumi}{\value{assumptions}}
\item \label{a:gen} There exists a limit function $q^\ast(\tau_1, \tau_2)$ such that $\frac{\Phi_{\mB}(\tau_1, \tau_2)}{n} \cip q^\ast(\tau_1, \tau_2)$ for all $\tau_1 \in [-\tau^\ast, \tau^\ast]$ and $\tau_2 \in [-1, 1]$. In addition, the partial derivatives of $q^\ast(\tau_1, \tau_2)$ exist at $\tau_1 = \tau_2 = 0$. Let them be denoted by  $\frac{\partial}{\partial \tau_1} q^\ast(0, 0) = \genvar^\ast$ and $\frac{\partial}{\partial \tau_2} q^\ast(0, 0) = \gencor^\ast$, respectively. We further assume that $\genvar^\ast \neq 0$.
\end{enumerate}

\begin{prop}\label{prop:gen}
Under Assumptions~\ref{a:Gaussian}--\ref{a:gen}, we have
\[
\gerrA \cip \gerrLim \quad \text{and} \quad \gerrB \cip \gerrLim,
\]
where
\[
\gerrLim \bydef \EE_{z_1, z_2}  \big[\fteacher(z_1) - {\fout}( \gencor^\ast z_1 + [\genvar^\ast - (\gencor^\ast)^2]^{1/2} z_2)\big]^2,
\]
and $z_1, z_2$ are two independent standard Gaussian random variables.

\end{prop}

\subsection{Related Work\label{subsec:relatedwork}}

The Gaussian equivalence phenomenon studied in this paper was stated in \cite{hastie2019surprises,mei2019generalization,montanari2019generalization,goldt2019modelling, Goldt2020Gaussian}, and explicitly exploited in \cite{montanari2019generalization,gerace2020generalisation,dhifallah2020precise,Dhifallah2021inherent} to derive the asymptotic limits of several learning problems. Related phenomena also appear in the context of random kernel matrices \cite{cheng2013spectrum,pennington2017nonlinear,louart2018random}, where it is shown that the impact of the nonlinear activation function [on the limiting singular value spectrum of the matrix $\mA$ in \eref{mat_AB}] can be captured by the three parameters in \eref{mu_constants}. However, these results on the asymptotic spectrum are not sufficient for our purpose. Except for the special case of ridge regression, the training and generalization errors of the learning problem in \eref{training} are not simple functions of the singular values/vectors of $\mA$. 

% \textcolor[rgb]{0.00,0.25,0.50}{A crucial step towards the rigorous justification of Gaussian equivalence phenomenon under more general settings is an interesting central limit theorem (CLT) type of results recently proved in \cite{Goldt2020Gaussian}.}
Recently, the authors of \cite{Goldt2020Gaussian} proved an interesting central limit theorem for the low-dimensional projections of $\va_t$ in \eref{a_vec} and $\vb_t$ in \eref{b_vec} onto generic low-dimensional subspaces. Specifically, for any $\vw \in \R^p$ with bounded $\ell_\infty$ norm and independent of $\va_t, \vb_t$, it is shown in \cite{Goldt2020Gaussian} that
\begin{equation}\label{eq:CLT_ind}
\big(\scp \va\tran_t \vw, \cvec\tran_t \sgl\big) \overset{\text{Law}}{\approx} \big(\scp\vb\tran_t \vw, \cvec\tran_t \sgl\big) \sim \mathcal{N}\Big(\mathbf{0}, \begin{bmatrix}\genvar & \pi\\ \gencor & 1 \end{bmatrix}\Big),
\end{equation}
where $\genvar= \vw\tran \mSig \vw / p$, with $\mSig$ defined in \eref{Sig}, and $\gencor = \mu_1 \sgl\tran \fmtx  \vw/{\sqrt{p}}$. This result is an important step towards a theoretical justification of the Gaussian equivalence, and indeed a quantitive version of \eref{CLT_ind} serves as a crucial ingredient of our proof. However, by itself the characterization in \eref{CLT_ind} does not imply the asymptotic equivalence stated in \eref{asymp_equiv}, as the training and generalization errors are all complicated functionals defined implicitly through the optimization problem \eref{training}. When calculating the generalization errors $\gerrA, \gerrB$ using \eref{gen_err}, for example, one will be dealing with two different weight vectors $\wt_{\mA}$ and $\wt_{\mB}$, respectively, as opposed to a single shared vector $\vw$ as in \eref{CLT_ind}. Showing that $\vw\tran_{\mA} \mSig \vw_{\mA} / p \approx \vw_{\mB}\tran \mSig \vw_{\mB} / p$ and $\sgl\tran \fmtx  \vw_{\mA}/{\sqrt{p}} \approx \sgl\tran \fmtx  \vw_{\mB}/{\sqrt{p}}$, which are the second-order statistics of the Gaussian distributions, is exactly among the technical challenges addressed in this work.

Our method for proving universality for the random feature model is based on the classical Lindeberg's principle \cite{lindeberg1922neue} and a leave-one-out analysis \cite{el2018impact} of the optimization problem in \eref{training}. Similar approaches have been used before to establish universality for various estimation problems \cite{oymak2018universality,korada2011applications,montanari2017universality,panahi2017universal,abbasi2019universality}. As a technical challenge in our problem, the entries of the regression vectors have a particular correlation structure, due to the presence of the random feature matrix $\fmtx$ in \eref{a_vec} and \eref{b_vec}. Thus, new techniques have to be developed to handle this correlation. Beyond the random feature model considered here, the Gaussian equivalence is a very general universality phenomenon that has been observed in many other models (see, \emph{e.g.}, \cite{Goldt2020Gaussian,seddik2020random,Dhifallah2021inherent,Loureiro2021capturing,gerace2022gaussian}).

\textcolor[rgb]{0.00,0.00,0.00}{After the initial release of this paper on arXiv, some of the results in this work have been used and adapted by other authors to rigorously establish the Gaussian equivalence phenomenon in several different settings.
Examples include minimum $\ell_1$ norm interpolated classification \cite{liang2020precise} and the feature learning in two-layer neural network \cite{ba2022high}.  
It will be interesting to extend the proof techniques in the current paper to handle some more general and challenging cases. Towards this direction, the recent paper \cite{montanari2022universality} by Montanari and Saeed studies the Gaussian equivalence of empirical risk minimization where the loss function and the regularizer do not need to be convex.}

% \textcolor[rgb]{0.00,0.50,1.00}{After the first version of this paper was posted, the results have been applied to rigorously establish the Guassian equivalence phenomenon in several settings such as minimum $\ell_1$ norm interpolated classification \cite{liang2020precise} and the asymptotics of feature learning \cite{ba2022high}. The recent paper \cite{montanari2022universality} by Montanari and Saeed studies the Gaussian equivalence of empirical risk minimization under a general feature map. Notably, their results apply to non-convex loss functions and regularizers.}

\textcolor[rgb]{0.00,0.00,0.00}{Finally, it is worth mentioning that all the aforementioned works focus on the so-called linear asymptotics regime, \emph{i.e,} $n/d\to\alpha$ and $p/d\to\eta$, where $\alpha,\eta\in(0,\infty)$. Recently, the Gaussian equivalence in the more general polynomial asymptotic regime, where $n/d^\ell\to\alpha\in(0,\infty)$, with $\ell\in\mathbb{Z}^{+}$, has been studied.
For example, the papers \cite{lu2022equivalence,misiakiewicz2022spectrum,xiao2022precise} analyze the spectrum of random inner-product matrices in the polynomial asymptotics regime, where $n/d^\ell\to\alpha\in(0,\infty)$, with $\ell\in\mathbb{Z}^{+}$. Based on these results, the exact learning performance of kernel ridge regression with polynomial scalings was established in \cite{misiakiewicz2022spectrum,hu2022sharp,xiao2022precise}.}

%As we mentioned above, the equivalence between the feature and Gaussian models can be viewed as a manifestation of the universality phenomenon, which has been observed in many high-dimensional estimation problems (see, \eg, \cite{donoho2009observed,korada2011applications,bayati2015universality,oymak2018universality,panahi2017universal,montanari2017universality,abbasi2019universality}). In the context of statistical learning, this phenomenon has been shown to exist in several popular models, including two-layer neural networks \cite{Goldt2020Gaussian} and generative adversarial nets (GAN) \cite{seddik2020random}. 


%In the context of compressed sensing, it is numerically observed \cite{donoho2009observed} that under several different sensing matrix ensembles, the probability of successful recovery undergoes phase transitions at the exactly same position. This intriguing phenomenon was then rigorously established in \cite{bayati2015universality} and \cite{oymak2018universality} under certain matrix ensembles with independent entries. In the other problem settings, such as LASSO \cite{,panahi2017universal}, Elastic Net \cite{montanari2017universality}, matrix recovery \cite{abbasi2019universality}, universality results are also proved when the underlying ensembles have independent entries.

\subsection{Paper Outline}

The rest of the paper is organized as follows.\ We prove Theorem~\ref{thm:get} and Proposition~\ref{prop:gen} in \sref{Proof-Sketch}. To emphasize readability, we only highlight the central ideas and key intermediate results there. In \sref{CLT}, we use Stein's method to provide an alternative proof of the central limit theorem for the nonlinear feature model. Heavier technical details are left to the appendix, where we compile all the auxiliary results. We conclude the paper in \sref{conclusion} with some additional remarks on how some of the technical assumptions in this work can be further relaxed.


==> Universality Laws for High-Dimensional Learning with Random Features_arXIv/proof_sketch.tex <==
%!TEX root = get_kernel.tex

\section{Proof of the Main Results}
\label{sec:Proof-Sketch}

\emph{Notation}: In our proof of Theorem~\ref{thm:get}, the parameters $\tau_1, \tau_2$ in \eref{gen_opt} are always kept fixed. Thus, to streamline the notation, we will write $\Phi_{\mA}(\tau_1, \tau_2)$ and $\Phi_{\mB}(\tau_1, \tau_2)$ simply as $\Phi_{\mA}$ and $\Phi_{\mB}$, when no confusion can arise. We will use $C$ and $c$ to denote generic constants that do not depend on the problem dimension $p$. To reduce the burden of bookkeeping, the exact values of $C$ and $c$ can change from one line to the next. In addition, $\polylog p$ stands for any function $B(p)$ that grows no faster than some polynomial of $\log p $, \ie,
\[
\abs{B(p)} \le C(1+\log^K\!p)
\]
for some finite $C > 0$ and $K \in \mathbb{Z}^+$. For a vector $\vx$, we use $\norm{\vx}$ to denote its 2-norm and $\norm{\vx}_\infty$ its $\ell_\infty$ norm. For a matrix $\mM$, its spectral and Frobenius norms are denoted by $\norm{\mM}$ and $\norm{\mM}_\text{F}$, respectively. Throughput the paper, we also adopt the following notational convention regarding conditional expectations. Given a family of independent random variables $X_1, X_2, \ldots, X_K$, we will write $\Ecnd{X_1}G(X_1, \ldots, X_K)$ for the conditional expectation of a function $G(\cdot)$ over $X_2, \ldots, X_K$, with $X_1$ kept fixed. A related notation is $\Eone{X_1}G(X_1, \ldots, X_K)$, where we take the expectation over $X_1$, conditional on all the other random variables. Finally, $\charfn_{\mathcal{A}}$ denotes the indicator function on a set $\mathcal{A}$, and $[n]$ stands for the set $\set{1, 2, \ldots, n}$.

\subsection{Test Functions}

We start by noting that, to prove the inequalities in \eref{get} and \eref{get2}, it suffices to show that
\begin{equation}\label{eq:test_func}
\begin{aligned}
        &\abs{\E \test(\tfrac{1}{p}{\Phi_{\mA}}) -  \E \test(\tfrac{1}{p}{\Phi_{\mB}})}  \\
    \le& \max\Big\{\norm{\test}_\infty, \norm{\test'}_\infty, \frac{\norm{\test''}_\infty}{\sqrt{p}}\Big\} \frac{\polylog p}{\sqrt{p}}
\end{aligned}
\end{equation}
for every bounded test function $\test(x)$ that also has bounded first and second derivatives. The precise connection between \eref{get}, \eref{get2} and \eref{test_func} will be made clear in \sref{get}, when we prove Theorem~\ref{thm:get}. For now, we focus on showing \eref{test_func}.

In our analysis, we first show a \emph{conditional} version of \eref{test_func}. Specifically, we will define a subset $\mathcal{A}$ of all $d \times p$ feature matrices, and show that
\begin{equation}\label{eq:cond_test}
\begin{aligned}
    &\sup_{\fmtx \in \mathcal{A}}\abs{\Ecnd{\fmtx}\test(\tfrac{1}{p}{\Phi_{\mA}})-  \Ecnd{\fmtx}\test(\tfrac{1}{p}{\Phi_{\mB}})} \\
    \le& \max\Big\{\norm{\test'}_\infty, \frac{\norm{\test''}_\infty}{\sqrt{p}}\Big\} \frac{\polylog p}{\sqrt{p}},
\end{aligned}
\end{equation}
where $\Ecnd{\fmtx}[\,\cdot\,]$ denotes the conditional expectation (over the input variables $\set{\cvec_i}$) for a fixed feature matrix $\fmtx$. We refer to $\mathcal{A}$ as the \emph{admissible set} of feature matrices, and its precise definition will be given in \sref{admissible}. To go from \eref{cond_test} to \eref{test_func}, we have
\begin{align}
&\abs{\EE \test(\tfrac{1}{p}{\Phi_{\mA}}) -  \EE \test(\tfrac{1}{p}{\Phi_{\mB}})} \nonumber \\
\le&  \EE\abs{\Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mA}})] -  \Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mB}})]}\nonumber\\
=&  \EE\abs{\Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mA}})] -  \Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mB}})]} (\charfn_{\mathcal{A}}(\fmtx) + \charfn_{\mathcal{A}^c}(\fmtx))\nonumber\\
\le& \sup_{\fmtx \in \mathcal{A}}\abs{\Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mA}})] -  \Ecnd{\fmtx}[\test(\tfrac{1}{p}{\Phi_{\mB}})]} + 2\norm{\test}_\infty \P(\mathcal{A}^c).
\label{eq:test_conditional_decomp}
\end{align}

The remaining tasks are now clear: (1) Establish \eref{cond_test}; and (2) show $\P(\mathcal{A}^c)  = \mathcal{O}(\polylog p / \sqrt{p})$. But first, we need to define the admissible set $\mathcal{A}$.

\subsection{The Admissible Set of Feature Matrices}
\label{sec:admissible}

Recall that $\fmtx = [\vf_1, \vf_2, \ldots, \vf_p]$, where $\set{\vf_i}_{i\in[p]}$ are the feature vectors. For notational simplicity, we add one more vector by letting $\vf_0 \bydef \sgl$. The admissible set $\mathcal{A}$ is constructed as
\begin{equation}\label{eq:def_setA}
\mathcal{A} = \mathcal{A}_1 \cap \mathcal{A}_2 \cap \mathcal{A}_3,
\end{equation}
where
\begin{align}
\label{eq:def_setA1}
\mathcal{A}_1 &\bydef \Big\{\fmtx \in \R^{d \times p}: \max_{0 \le i \le j \le p} \abs{\vf_i\tran \vf_j - \delta_{ij}}\le \tfrac{(\log p)^2}{\sqrt{p}}\Big\}, \\
\intertext{with $\delta_{ij}$ denoting the Kronecker delta function, and}
%, \max_{0 \le i < j \le p} \abs{\vf_i \vf_j} \le \tfrac{C[(\log p)^2+1]}{\sqrt{p}}}\\
%\mathcal{A}_2 &\bydef \set{\fmtx \in \R^{d \times p}: \max_{0 \le i < j \le p} \abs{\vf_i \vf_j} \le \frac{\polylog p}{\sqrt{p}}}\\ \intertext{and}
\mathcal{A}_2 &\bydef \set{\fmtx \in \R^{d \times p}: \norm{\fmtx} \le 1+2\sqrt{\eta} },\label{eq:def_setA2}
\end{align}
where $\eta$ is the constant in Assumption~\ref{a:dimensions}. Before defining $\mathcal{A}_3$, which requires some additional notation, we first note that $\mathcal{A}_1 \text{ and } \mathcal{A}_2$ are all high-probability events under Assumption~\ref{a:feature}. Specifically, standard concentration inequalities for sub-Gaussian random vectors give us
\begin{equation}\label{eq:A1A2_p}
\P(\mathcal{A}_1) \ge 1 - ce^{-\left(\log p\right)^{2}/c}
\end{equation}
for some $c > 0$. (See Lemma~\ref{lem:A1_high_prob} in Appendix~\ref{appendix:Concentration-of-GaussianVec} for a proof.) Similarly, applying matrix concentration inequalities [\eqref{eq:spectral_norm_Wishart} in Appendix~\ref{appendix:matrix}], we can conclude that
\begin{equation}\label{eq:A3_p}%
\P(\mathcal{A}_2) \ge 1 - 2 e^{-cp}
\end{equation}
for some constant $c>0$.

The definition of the last set $\mathcal{A}_3$ in \eref{def_setA} is a bit technical. Consider a family of optimization problems
\begin{align}
\Phi_{k}\bydef & \min_{\vw\in\R^{p}}\Big\{\textstyle\sum_{t=1}^{k}\loss(\tfrac{1}{\sqrt{p}}\vb_{t}\tran\vw;y_{t})+\sum_{t=k+1}^{n}\loss(\tfrac{1}{\sqrt{p}}\va_{t}\tran\vw;y_{t})\nonumber \\
&\hspace{2.8em}+\sum_{j=1}^{p}\regu(w_{j})+Q(\vw)\Big\},\label{eq:interpolation_k}\\
\wt_{k}\bydef & \argmin{\vw\in\R^{p}}\Big\{\textstyle\sum_{t=1}^{k}\loss(\tfrac{1}{\sqrt{p}}\vb_{t}\tran\vw;y_{t})+\sum_{t=k+1}^{n}\loss(\tfrac{1}{\sqrt{p}}\va_{t}\tran\vw;y_{t}) \nonumber\\
&\hspace{3.9em}+\sum_{j=1}^{p}\regu(w_{j})+Q(\vw)\Big\},\label{eq:interpolation_k_wt}
\end{align}
for $0 \le k \le n$, where $\set{\va_\didx}$ and $\set{\vb_\didx}$ are the regressors in \eref{a_vec} and \eref{b_vec}, respectively, and
\begin{align}
\label{eq:Q_def}
Q(\vw) \bydef {\tau_1} \vw\tran \mSig \vw + \tau_2\mu_1\sqrt{p} \sgl\tran \fmtx \vw.
\end{align}
The reason for considering this sequence of problems will become clear in \sref{Lindeberg}. For now, just note that our quantities of interest, namely $\Phi_{\mA}$ and $\Phi_{\mB}$, are just the starting and end point of this sequence, \ie, $\Phi_{0}=\Phi_{\mA}$ and $\Phi_{n}=\Phi_{\mB}$. We then have
\begin{align}
\label{eq:def_setA3}
\mathcal{A}_3 \bydef  \Big\{\fmtx \in \R^{d \times p}: \Big[\max_{0 \le k \le n} \Ecnd{\fmtx}\norm{\wt_k}_\infty^2\Big] \le \left(\log p\right)^{7+4K_1}\Big\},
\end{align}
where $K_1$ is the constant in Assumption~\ref{a:loss}.
\begin{prop}\label{prop:wt_bnd}
Under Assumptions~\ref{a:Gaussian}--\ref{a:feature}, there exists some $c>0$ such that
\begin{equation}\label{eq:A4_p}
\P({\cal A}_{3})\geq 1-c e^{-\left(\log p\right)^{2}/c}.
\end{equation}
\end{prop}
This result, whose proof can be found in Appendix~\ref{appendix:linfty_boundedness}, shows that $\mathcal{A}_3$ is still a high-probability event. In light of \eref{A1A2_p}, \eref{A3_p} and \eref{A4_p}, there exists $c>0$ such that
\begin{align}
\label{eq:A_small_prob}
\P(\mathcal{A}^c) \le \P(\mathcal{A}_1^c) + \P(\mathcal{A}_2^c) + \P(\mathcal{A}_3^c) \le  ce^{-\left(\log p\right)^{2}/c}.
\end{align}

\subsection{The Lindeberg Method}
\label{sec:Lindeberg}

%In this section, we will consider the conditional expectation over a given $\fmtx\in\cal{A}$.
%%To lighten notation, we will not write explicitly $\E(\cdot \mid \fmtx)$, but simply denote it as $\E(\cdot)$.
%The reason for us to consider the conditional expectation has been explained in \eqref{eq:test_conditional_decomp}.

In what follows, we prove \eref{cond_test} by using Lindeberg's method \cite{lindeberg1922neue,korada2011applications,panahi2017universal}.
The idea is simple: The sequence shown in \eqref{eq:interpolation_k} serves as an interpolation path that allows us to go from $\Phi_{\mA}$ to $\Phi_{\mB}$. To prove \eref{cond_test}, it suffices to show that the difference between any two neighboring
points on the interpolation path is small. Indeed, as there are only $n = \mathcal{O}(p)$ such pairwise comparisons, we just need to show that
\[
\abs{\Ecnd{\fmtx} \big[\test\big(\tfrac{1}{p}\Phi_{k}\big)\big]-\Ecnd{\fmtx}\big[ \test\big(\tfrac{1}{p}\Phi_{k-1}\big)\big]} = \mathcal{O}\Big(\frac{\polylog p}{p^{3/2}}\Big),
\]
uniformly over $\fmtx \in \mathcal{A}$ and $1 \le k \le n$.

By construction, the optimization problems associated with $\Phi_k$ and $\Phi_{k-1}$ differ only in their choice of the $k$th regressor. The former uses $\vb_k$, whereas the latter uses $\va_k$. Consequently, both $\Phi_k$ and $\Phi_{k-1}$ can be seen as a perturbation of a common ``leave-one-out'' problem:
\begin{align}
\label{eq:LOO_objctive_function}
\Phi_{\bs k}\bydef & \min_{\vw\in\R^p} \big\{\textstyle\sum_{t=1}^{k-1}\loss(\tfrac{1}{\sqrt{p}}\vb_{t}\tran\vw;y_{t})+\sum_{t=k+1}^{n}\loss(\tfrac{1}{\sqrt{p}}\va_{t}\tran\vw;y_{t}) \nonumber \\
&\hspace{3em}+\sum_{j=1}^{p}\regu(w_{j})+Q(\vw)\big\}.
\end{align}
As $\Phi_k \approx \Phi_{\bs k}$, it is natural to apply Taylor's expansion around $\Phi_{\bs k}$, which gives us
\begin{equation}\label{eq:phik_expansion}
\begin{aligned}
    \test(\tfrac{1}{p}\Phi_{k}) =& \test(\tfrac{1}{p}\Phi_{\bs k}) + \tfrac{1}{p} \test'(\tfrac{1}{p}\Phi_{\bs k}) ({\Phi_{k}} - {\Phi_{\bs k}}) \nonumber \\
    &+ \tfrac{1}{2p^2} \test''(\theta) ({\Phi_{k}} - {\Phi_{\bs k}})^2,
\end{aligned}
\end{equation}
with $\theta$ denoting some value that lies between $\tfrac{1}{p}\Phi_{k}$ and $\tfrac{1}{p}\Phi_{\bs k}$. Writing an analogous expansion for $\btest(\Phi_{k-1})$ around $\Phi_{\bs k}$, and then subtracting it from \eref{phik_expansion}, we can get
\begin{equation}\label{eq:testfunc_interpolation}
\begin{aligned}
&\left|\Ecnd{\fmtx}\big[ \test\big(\tfrac{1}{p}\Phi_{k}\big)\big]-\Ecnd{\fmtx}\big[ \test\big(\tfrac{1}{p}\Phi_{k-1}\big)\big]\right| \\
\le&  \tfrac{\left\Vert \test'(x)\right\Vert _{\infty}}{p}\Ecnd{\fmtx}\left|\E_{k}\left(\Phi_{k}-\Phi_{k-1}\right)\right|\\
 &+\tfrac{\left\Vert \test''(x)\right\Vert _{\infty}}{2p^{2}}\left[\Ecnd{\fmtx}\left(\Phi_{k}-\Phi_{\bs k}\right)^{2}+\Ecnd{\fmtx}\left(\Phi_{k-1}-\Phi_{\bs k}\right)^{2}\right],
\end{aligned}
\end{equation}
where $\E_k$ denotes the conditional expectation over the random vectors $\{\va_k, \vb_k\}$ associated with the $k$th training sample, while keeping everything else, \ie, $\{\va_t, \vb_t\}_{t\neq k}$ and $\fmtx$, fixed.

To make further progress, we need to introduce a surrogate optimization problem:
\begin{equation}\label{eq:quadratic_approx_objctive_function}
\begin{aligned}
    \Psi_{k}(\vr)\bydef&
    \Phi_{\bs k}+\min_{\vw\in\R^p}\Big\{\frac{1}{2}(\vw-\loowt{\bs k})\tran\mH_{\bs k}(\vw-\loowt{\bs k}) \\
    &\hspace{6em}+\loss(\tfrac{1}{\sqrt{p}}\vr\tran\vw;y_{k})\Big\},
\end{aligned}
\end{equation}
where $\loowt{\bs k}$ is the leave-one-out optimal solution of \eqref{eq:LOO_objctive_function}, and
\begin{equation}\label{eq:looH}
\begin{aligned}
\mH_{\bs k} \bydef& \frac{1}{p}\textstyle\sum_{t=1}^{k-1}\loss''(\tfrac{1}{\sqrt{p}}\vb_{t}\tran\loowt{\bs k};y_{t})\vb_{t}\vb_{t}\tran \\
&+\displaystyle\frac{1}{p}\textstyle\sum_{t=k+1}^{n}\loss''(\tfrac{1}{\sqrt{p}}\va_{t}\tran\loowt{\bs k};y_{t})\va_{t}\va_{t}\tran\\
&+\diag\Big\{ h''\big(w_{\bs k,i}^{*}\big)\Big\} +\nabla^{2}Q(\loowt{\bs k})
\end{aligned}
\end{equation}
is the Hessian matrix of the objective function in \eref{LOO_objctive_function} evaluated at $\loowt{\bs k}$. We note that $\Psi_k(\vr)$ has a simple interpretation: By setting $\vr = \vb_k$, we can see that the optimization problem associated with $\Psi_k(\vb_k)$ is simply a quadratic approximation of the one associated with $\Phi_k$ in \eref{interpolation_k}. Similarly, $\Psi_k(\va_k)$ is a quadratic approximation of $\Phi_{k-1}$. The following lemma, whose proof can be found in Appendix~\ref{appendix:quad_approx}, quantifies the accuracy of such approximation.
\begin{lem}
\label{lem:quad_approx}We have
\begin{equation}\label{eq:quad_approx_psi_phi_k}
\begin{aligned}
   &\max\{\Ecnd{\fmtx}\left(\Psi_{k}(\vb_k) - \Phi_{\bs k}\right)^2,\Ecnd{\fmtx}\left(\Psi_{k}(\va_k) - \Phi_{\bs k}\right)^2\} \\
   \leq& \polylog p, 
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:quad_approx_phi_psi}
\begin{aligned}
    &\max\set{\Ecnd{\fmtx}\left(\Psi_{k}(\vb_k)-\Phi_{k}\right)^2,\Ecnd{\fmtx}\left(\Psi_{k}(\va_k)-\Phi_{k-1}\right)^2} \\
    \leq& \frac{\polylog p}{p},
\end{aligned}
\end{equation}
both of which hold uniformly over $\fmtx\in \mathcal{A}$ and $k\in[n]$.
\end{lem}

% and second-order approximate solution as $\qwt$.
%Then the difference $\left|\E g\left(\frac{\Phi_{k}}{p}\right)-\E g\left(\frac{\Phi_{k-1}}{p}\right)\right|$ between neighbouring
%points on the interpolation path can be bounded in terms of $\Phi_{k-1}$, $\Phi_{k}$ and $\Phi_{\bs k}$ as follows.

%We can approximate $\test\left(\tfrac{1}{p}\Phi_{k-1}\right)$ in the same way.

%A key step in the proof is splitting $\left|\E g\left(\frac{\Phi_{k}}{p}\right)-\E g\left(\frac{\Phi_{k-1}}{p}\right)\right|$ as:
%\begin{align*}
%&\left|\E g\left(\frac{\Phi_{k}}{p}\right)-\E g\left(\frac{\Phi_{k-1}}{p}\right)\right|\\
%\leq &\left|\E g\left(\frac{\Phi_{k}}{p}\right)-\E g\left(\frac{\Psi_{k}}{p}\right)\right|
%+\left|\E g\left(\frac{\Psi_{k}}{p}\right)-\E g\left(\frac{\Psi_{k-1}}{p}\right)\right|
%+\left|\E g\left(\frac{\Psi_{k-1}}{p}\right)-\E g\left(\frac{\Phi_{k-1}}{p}\right)\right|,
%\end{align*}

Using this lemma, we can now bound the terms on the right-hand side of \eqref{eq:testfunc_interpolation} as follows:
\begin{align}
\label{eq:quad_decomp_1}
&\Ecnd{\fmtx}\left|\E_{k}\left(\Phi_{k}-\Phi_{k-1}\right)\right| \nonumber \\
\le& \Ecnd{\fmtx}\absb{\E_{k}[\Psi_{k}(\vb_k)-\Psi_{k}(\va_k)]} + \Ecnd{\fmtx}\left|\Psi_{k}(\vb_k)-\Phi_{k}\right| \nonumber \\
&+\Ecnd{\fmtx}\left|\Psi_{k}(\va_k)-\Phi_{k-1}\right|\nonumber\\
\le&  \Ecnd{\fmtx}\absb{\E_{k}[\Psi_{k}(\vb_k)-\Psi_{k}(\va_k)]} + \polylog p / \sqrt{p},
\end{align}
where to reach the last step we have used H\"{o}lder's inequality and \eref{quad_approx_phi_psi}. Meanwhile, combining \eref{quad_approx_phi_psi} and \eref{quad_approx_psi_phi_k} gives us
\begin{equation}\label{eq:quad_decomp_2}
\begin{aligned}
    &\Ecnd{\fmtx}\left(\Phi_{k}-\Phi_{\bs k}\right)^{2} \\ \leq& 2\Ecnd{\fmtx}\left(\Phi_{k}-\Psi_{k}(\vb_k)\right)^{2} + 2\Ecnd{\fmtx}\left(\Psi_{k}(\vb_k)-\Phi_{\bs k}\right)^{2} \\
    \le& \polylog p,
\end{aligned}
\end{equation}
and similarly,
\begin{equation}\label{eq:quad_decomp_3}
\Ecnd{\fmtx}\left(\Phi_{k-1}-\Phi_{\bs k}\right)^{2} \le \polylog p.
\end{equation}
In light of \eref{quad_decomp_1}, \eref{quad_decomp_2}, and \eref{quad_decomp_3}, we just need to show that
\[
\Ecnd{\fmtx}\absb{\E_{k}[\Psi_{k}(\vb_k)-\Psi_{k}(\va_k)]} = o(1)
\]
to get a useful bound for the left-hand side of \eref{testfunc_interpolation}.

We are now in a position to show why we introduce and work with $\Psi_k(\vr)$. Let $\calM_{k}(x;\gamma)$ denote the \emph{Moreau envelope} of the loss function
$\loss\left(x;y_{k}\right)$, \ie,
\begin{equation}\label{eq:Moreau_envelope}
\calM_{k}(x;\gamma)\bydef\min_{z}\Big\{\loss\left(z;y_{k}\right)+\frac{(x-z)^{2}}{2\gamma}\Big\},
\end{equation}
where $\gamma > 0$ is some fixed parameter. It is straightforward to show (see Lemma~\ref{lem:quadapprox_optsol} in Appendix~\ref{appendix:opt_properties}) that
\begin{equation}\label{eq:Rk_cr_decomp_general}
\Psi_{k}(\vr)=\Phi_{\bs k}+\calM_{k}\big(\scp{\vr\tran\loowt{\bs k}};\gamma_{k}(\vr)\big),
\end{equation}
where
\begin{equation}\label{eq:gamma_k}
\gamma_{k}(\vr)\bydef({\vr\tran\mH_{\bs k}^{-1}\vr})/{p}.
\end{equation}
It then follows that
\begin{equation}\label{eq:Moreau_diff}
\begin{aligned}
    \Psi_k(\vb_k) - \Psi_k(\va_k) =& \calM_{k}\big(\scp{\vb_k\tran\loowt{\bs k}};\gamma_{k}(\vb_k)\big) \nonumber \\
    &- \calM_{k}\big(\scp{\va_k\tran\loowt{\bs k}};\gamma_{k}(\va_k)\big).
\end{aligned}
\end{equation}
By construction, both $\va_k$ and $\vb_k$ are independent of the leave-one-out solution $\loowt{\bs k}$ and the Hessian matrix $\mH_{\bs k}$. It is this independent structure that significantly simplifies our analysis.

As $p \to \infty$, the scalars $\gamma_{k}(\vb_k)$ and $\gamma_{k}(\va_k)$ in \eref{Moreau_diff} concentrate around a common value $\gamma_k \bydef  \E_{k}\gamma_{k}(\vb_{k})$. This then prompts us to write the following decomposition
\begin{equation}\label{eq:Phi_k_decomp_2}
\begin{aligned}
 &\Ecnd{\fmtx}\left|\E_{k}(\Psi_{k}(\vb_k)-\Psi_{k}(\va_k))\right|\\
  \le& \Ecnd{\fmtx}\underbrace{\absb{\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\vb_{k}\tran\loowt{\bs k};\gamma_{k}\big)-\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\va_{k}\tran\loowt{\bs k};\gamma_{k}\big)}}_{\Delta_{\text{CLT}}} \\
  &+ \Delta_1 + \Delta_2,
 \end{aligned}
\end{equation}
where
\begin{equation}\label{eq:Phi_decomp_D1}
\begin{aligned}
    &\Delta_1  
    \bydef \Ecnd{\fmtx}\absb{\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\vb_{k}\tran\loowt{\bs k};\gamma_{k}(\vb_{k})\big) \\
    &\hspace{11em}-\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\vb_{k}\tran\loowt{\bs k};\gamma_{k}\big)}
\end{aligned}
\end{equation}
and
\begin{equation}\label{eq:Phi_decomp_D2}
\begin{aligned}
    &\Delta_2 
    \bydef\Ecnd{\fmtx}\absb{\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\va_{k}\tran\loowt{\bs k};\gamma_{k}(\va_{k})\big) \\
    &\hspace{11em}-\E_{k}\calM_{k}\big(\tfrac{1}{\sqrt{p}}\va_{k}\tran\loowt{\bs k};\gamma_k\big)}.
\end{aligned}
\end{equation}
These last two terms are easy to control, due to the concentrations of $\gamma_{k}(\vb_k)$ and $\gamma_{k}(\va_k)$ around $\gamma_k$. As shown in Lemma~\ref{lem:pathdiff_D1D2_bd} in Appendix~\ref{appendix:Thm2_satisfy}, we have
\begin{equation}\label{eq:D1D2_max}
\max\set{\Delta_1, \Delta_2} \le \frac{\polylog p}{\sqrt{p}},
\end{equation}
uniformly over $\fmtx \in \mathcal{A}$ and $k\in [n]$.



%and control each term on the RHS, which can be done in the same way.
%\begin{lem}
%\label{lem:testfn_bd}
%\end{lem}

%The proof of Lemma \ref{lem:testfn_bd} will be given in Section \ref{}. From (\ref{eq:testfunc_interpolation}), we know
%it suffices to show $\E_{\bs k}\left|\E_{k}\left(\Phi_{k}-\Phi_{k-1}\right)\right|\sim o\left(1\right)$,
%$\E\left(\Phi_{k-1}-\Phi_{\bs k}\right)^{2}\sim\calO(1)$ and $\E\left(\Phi_{k}-\Phi_{\bs k}\right)^{2}\sim\calO(1)$.

%A key step to analyze these difference terms $\Phi_{k}-\Phi_{k-1}$ and $\Phi_{k}-\Phi_{\bs k}$ is to consider their quadratic approximations.
%Note that $\objfn_{k}(\vw;\vr)=\objfn_{k}(\vw;\boldsymbol{0})+\loss(\tfrac{1}{\sqrt{p}}\vr\tran\vw;y_{k})$,
%so $\Phi_{k}$ and $\Phi_{k-1}$ are small perturbations
%around $\Phi_{\bs k}$ by adding a single loss term associated with
%the new observation $\left(\vr,y_{k}\right)$. Therefore, we can consider
%the following second order approximation of $\objfn_{k}(\vw;\vr)$ near $\loowt{\bs k}$:


%Correspondingly, we define
%\begin{equation}
%\Psi_{k}\bydef\min_{\vw\in\R^{p}}S_{k}(\vw;\vb_{k}),\qquad\Psi_{k-1}\bydef\min_{\vw\in\R^{p}}S_{k}(\vw;\va_{k}).\label{eq:quadratic_approximation_opt}
%\end{equation}

%In the sequel, we will separately bound $\E\left(\Psi_{k}-\Phi_{\bs k}\right)^{2}$, $\E_{k}\left(\Phi_{k}-\Psi_{k}\right)^2$
%and $\left|\E_{k}\left(\Psi_{k}-\Psi_{k-1}\right)\right|$.

It is more challenging to bound the term $\Delta_\text{CLT}$, whose subscript alludes to the fact that we will be using a version of the central limit theorem. To see that, we first recall from \eref{Moreau_envelope} that the Moreau envelope $\calM_{k}(x;\gamma_k)$ depends on the training label $y_k$. The latter is generated by the model in \eref{teacher}, with a teacher function $\fteacher(x)$. Introducing a two-dimensional test function
\begin{equation}\label{eq:test_M}
\btest(x; s) \bydef\min_{z}\loss\left(z;\fteacher(s)\right)+\frac{(x-z)^{2}}{2\gamma_k},
\end{equation}
we can then write
\[
\Delta_\text{CLT} = \absb{\E_{k}\btest\big(\tfrac{1}{\sqrt{p}}\va_{k}\tran\loowt{\bs k};\cvec_k\tran \sgl\big)-\E_{k}\btest\big(\tfrac{1}{\sqrt{p}}\vb_{k}\tran\loowt{\bs k};\cvec_k\tran \sgl\big)}.
\]
That $\Delta_\text{CLT} = o(1)$ is due to the following fact: When conditioned on $\fmtx$ and $\loowt{\bs k}$, we have
\begin{equation}
\label{eq:clt_informal}
\big(\scp{\va\tran_k \loowt{\bs k}}, \cvec_k\tran \sgl\big) \overset{\text{Law}}{\approx} \big(\scp{\vb_k\tran \loowt{\bs k}}, \cvec_k\tran \sgl\big) \sim \text{jointly Gaussian}.
\end{equation}
Making \eqref{eq:clt_informal} precise is the focus of Theorem~\ref{thm:CLT_general} in \sref{CLT}. It is easy to verify that the test function defined in \eref{test_M} indeed satisfies the assumptions of Theorem~\ref{thm:CLT_general}. (See Lemma~\ref{lem:Thm2_satisfy} in Appendix~\ref{appendix:Thm2_satisfy}.) Consequently, for every $\fmtx \in \mathcal{A}$, Theorem~\ref{thm:CLT_general} gives us
\begin{align}
&\Ecnd{\fmtx} [\Delta_\text{CLT}] \nonumber\\
\overset{(a)}{\le}&  \Ecnd{\fmtx} \big[(1 + \norm{\loowt{\bs k}}_\infty [1+\BPf])(1 + (\scp\norm{\loowt{\bs k}})^{K})\big]\frac{\polylog p}{\sqrt{p}}\nonumber\\
\le&  \Ecnd{\fmtx} \big[1 + (1+\BPf)^2 \norm{\loowt{\bs k}}_\infty^2 + (\scp\norm{\loowt{\bs k}})^{2K}\big]\frac{\polylog p}{\sqrt{p}}\nonumber\\
\overset{(b)}{\le}& \frac{\polylog p}{\sqrt{p}}.\label{eq:D_clt}
\end{align}
In (a), $\BP$ is the bound in \eref{BP}, and $K$ is some positive constant. To reach (b), we have used the fact that $\fmtx \in \mathcal{A}_2$, which then implies that $\BP \le \polylog p$, and $\fmtx \in \mathcal{A}_3$, which guarantees the boundedness of $\Ecnd{\fmtx} \norm{\loowt{\bs k}}_\infty^2$. Finally, the boundedness of $\Ecnd{\fmtx}(\scp\norm{\loowt{\bs k}})^{2K}$ is verified in Lemma \ref{lem:norm_optwt_Expec_bd_A2}.

We can now retrace our steps to reach our goal of proving \eref{cond_test}. Specifically, substituting \eref{D_clt} and \eref{D1D2_max} into \eref{Phi_k_decomp_2} gives us $\Ecnd{\fmtx}\absb{\E_{k}(\Psi_{k}(\vb_k)-\Psi_{k}(\va_k))} \le \polylog p / \sqrt{p}$, which, together with \eref{quad_decomp_1}, \eref{quad_decomp_2}, \eref{quad_decomp_3}, and \eref{testfunc_interpolation}, leads to
\begin{equation}\label{eq:cond_test_k}
\begin{aligned}
    &\absb{\Ecnd{\fmtx}\big[ \test\big(\tfrac{1}{p}\Phi_{k}\big))\big]-\Ecnd{\fmtx}\big[ \test\big(\tfrac{1}{p}\Phi_{k-1}\big)\big]} \\
&\hspace{2.8em} \le  \max\Big\{\left\Vert \test'(x)\right\Vert _{\infty}, \frac{\left\Vert \test''(x)\right\Vert _{\infty}}{\sqrt{p}}\Big\}\frac{\polylog p}{p^{3/2}}.
\end{aligned}
\end{equation}
Note that the upper bound is uniform over all $\fmtx \in \mathcal{A}$ and all $k \in [n]$. Now let us recall the construction of the interpolation sequence in \eref{interpolation_k}. Since $\Phi_{0}=\Phi_{\mA}$ and $\Phi_{n}=\Phi_{\mB}$, we obtain \eref{cond_test} from \eref{cond_test_k} via triangle inequality. Finally, given the decomposition in \eref{test_conditional_decomp} and the probability bound in \eref{A_small_prob}, we establish the inequality in \eref{test_func}.

Before proceeding to the proof of Theorem~\ref{thm:get}, we pause and point out a subtle issue regarding the central limit theorem stated informally in \eref{clt_informal}. It is important that the weight vector in \eref{clt_informal} is the leave-one-out solution $\loowt{\bs k}$, which is independent of both $\va_k$ and $\vb_k$. The situation will be very different if we use the original optimal solution $\wt_{k}$ instead.
In this case, the asymptotic distribution of $\scp{\va\tran_k \wt_{k}}$ is not Gaussian (\emph{i.e.}, the central limit theorem is no longer valid), due to the weak yet non-negligible correlation between $\wt_{k}$ and $\va_k$.We illustrate this fact in Fig. \ref{fig:Empirical-distributions-of}. The theoretical prediction of the limit distributions shown in the figure can be found by using Lemma \ref{lem:quadapprox_optsol} and Lemma \ref{lem:qwt_wt_deterministic_bd} in Appendix \ref{appendix:opt_properties}.
\begin{figure*}[t]
\begin{centering}
\subfigure[$\lambda=1$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_1_1}
\par\end{centering}

}\hphantom{}\subfigure[$\lambda=10^{-2}$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_2_1}
\par\end{centering}

}\hphantom{}\subfigure[$\lambda=10^{-3}$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_3_1}
\par\end{centering}
}
\par\end{centering}
\begin{centering}
\subfigure[$\lambda=1$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_1_2}
\par\end{centering}
}\hphantom{}\subfigure[$\lambda=10^{-2}$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_2_2}
\par\end{centering}
}\hphantom{}\subfigure[$\lambda=10^{-3}$]{\begin{centering}
\includegraphics[scale=0.32]{fig/histogram_3_2}
\par\end{centering}
}
\par\end{centering}
\caption{Empirical distributions of $\scp{\va\tran_k \wt_{k}}$,
{[}(a)-(c){]} and $\scp{y_k\va\tran_k \wt_{k}}$,
{[}(d)-(f){]}. Here $\kernel(x) = \tanh(x)$, $\ell(x; y)$ is the logistic loss, $h(x)=\tfrac{\lambda}{2}x^2$, and $\fteacher(x) = \fout(x) = \sign(x)$. We fix $d=600$, $p=900$ and $n=1800$, while considering three different values of $\lambda$. The histograms are plotted on the values
of $\{\scp{\va\tran_k \wt_{k}}\}_{k\in[n]}$ and $\{\scp{y_k\va\tran_k \wt_{k}}\}_{k\in[n]}$
from 10 independent runs.  The dashed lines show Gaussian PDFs with the same empirical means and variances of the histograms. Observe that the empirical distributions of $\{\scp{\va\tran_k \wt_{k}}\}_{k\in[n]}$ and $\{\scp{y_k\va\tran_k \wt_{k}}\}_{k\in[n]}$ are not Gaussian, and the difference becomes increasing noticeable as $\lambda$ becomes smaller. The correct limit distributions are obtained by using Lemma \ref{lem:quadapprox_optsol} and Lemma \ref{lem:qwt_wt_deterministic_bd}.\label{fig:Empirical-distributions-of}}
\end{figure*}


\subsection{Proof of Theorem~\ref{thm:get}}
\label{sec:get}

Equipped with \eref{test_func}, we just need to construct a suitable test function in order to complete the proof. For any fixed $\veps>0$ and $c$, let
\begin{equation}
\test_{\veps}(x)=(\charfn_{|x|\geq3\veps/2}*\mol_{\veps/2})(x-c),\label{eq:smoothed_test_fn}
\end{equation}
where $\mol_{\veps/2}(x)$ is a scaled mollifier defined in \eref{sc_mol} in Appendix \ref{appendix:truncation}. By properties of $\mol_{\veps/2}(x)$, it is easy to check that $\norm{\test_{\veps}'}_{\infty}<{C}/{\veps}$ and $\norm{\test_{\veps}''}_{\infty}<{C}/{\veps^{2}}$. Moreover,
\begin{equation}\label{eq:smoothed_test_fn_bd}
\charfn_{|x-c|\geq 2\veps}\leq\test_{\veps}(x)\leq\charfn_{|x-c|\geq\veps}.
\end{equation}
Letting $x = \Phi_{\mA}/p$ and taking expectation over the functions in \eref{smoothed_test_fn_bd}, we have
\[
P(\abs{\Phi_{\mA}/p-c}\ge2\varepsilon)\le\E\test_{\veps}(\Phi_{\mA}/p).
\]
Changing $x$ to $\Phi_{\mB}/p$ yields
\[
\E\test_{\veps}(\Phi_{\mB}/p) \le P(\abs{\Phi_{\mB}/p-c}\ge \varepsilon).
\]
Applying \eref{test_func}, we then have
\begin{align*}
    P(\abs{\Phi_{\mA}/p-c}\ge2\varepsilon)\le P(\abs{\Phi_{\mB}/p-c}\ge \varepsilon) &\\
&\hspace{-8em}+ \max\Big\{\veps, 1, \frac{1}{\veps\sqrt{p}}\Big\} \frac{\polylog p}{\veps\sqrt{p}},
\end{align*}
which leads to \eref{get} for $\veps \in (0, 1)$ and $p\geq \tfrac{1}{\veps^2}$. The proof of \eref{get2} is analogous, as the above procedure is completely symmetric with respect to $\Phi_{\mA}$ and $\Phi_{\mB}$.


\subsection{Proof of Proposition~\ref{prop:gen}}
\label{sec:proof_gen}

Let $\cvec_\text{new} \sim \mathcal{N}(0, \mI_d)$ be a Gaussian vector independent of the existing training samples and the feature matrix. Substituting \eref{teacher} into \eref{gen_err}, we can then write the generalization errors as
\[
\gerrA = \Eone{\cvec_\text{new}}[\fteacher(\cvec_\text{new}\tran \sgl) - \fout(\scp \va_\text{new}\tran \wt_{\mA})]^2
\]
and
\[
\gerrB = \Eone{\cvec_\text{new}}[\fteacher(\cvec_\text{new}\tran \sgl) - \fout(\scp \vb_\text{new}\tran \wt_{\mB})]^2,
\]
respectively. Here, $\va_\text{new} = \kernel(\fmtx\tran \cvec_\text{new})$ and $\vb_\text{new} = \mu_1 \fmtx\tran \cvec_\text{new} + \mu_2 \vz_\text{new}$, where $\vz_\text{new} \sim \mathcal{N}(0, \mI_p)$ is an independent Gaussian vector. Note that $(\cvec_\text{new}\tran \sgl, \scp \vb_\text{new}\tran \wt_{\mB})$ are jointly Gaussian, and thus their distributions are completely determined by their covariance matrix. As $\norm{\sgl} = 1$, we have $\E (\cvec_\text{new}\tran \sgl)^2 = 1$. Let $\genvar_B \bydef \E (\scp \vb_\text{new}\tran \wt_{\mB})^2$ and $\gencor_B \bydef \E (\cvec_\text{new}\tran \sgl) (\scp \vb_\text{new}\tran \wt_{\mB})$. Clearly,
\begin{equation}\label{eq:genvar}
\genvar_B = \frac{[\wt_{\mB}]\tran \mSig \wt_{\mB}}{p} \quad \text{and} \quad \gencor_B = \frac{\mu_1 \sgl\tran \fmtx  \wt_{\mB}}{\sqrt{p}},
\end{equation}
where $\mSig$ is the matrix in \eref{Sig}. It is also easy to check that $\gerrB = G(\genvar_B, \gencor_B)$, where
\begin{equation}\label{eq:G_func}
G(\genvar, \gencor) \bydef \E_{z_1, z_2} [\fteacher(z_1) - \fout(\gencor z_1 + [{\genvar - \gencor^2}]^{1/2} z_2)]^2,
\end{equation}
with $z_1, z_2 \overset{\text{i.i.d.}}{\sim}{\mathcal{N}(0, 1)}$.

The rest of the proof falls naturally into three parts: (a) We will first show that $\genvar_B \to \genvar^\ast = \frac{\partial}{\partial \tau_1} q^\ast(0, 0)$ and $\gencor_B \to \gencor^\ast = \frac{\partial}{\partial \tau_2} q^\ast(0, 0)$, where $q^\ast(\tau_1, \tau_2)$ is the limit function in Assumption~\ref{a:gen}; (b) By replacing $\wt_{\mB}$ in \eref{genvar} with $\wt_{\mA}$, we introduce the analogous quantities $\genvar_A$ and $\gencor_A$. We will show that $\genvar_A, \gencor_A$ have the same limits as $\genvar_B, \gencor_B$; (c) Finally, we will show that $\gerrA \approx G(\genvar_A, \gencor_A)$ with high probability, where $G(\cdot, \cdot)$ is the function in \eref{G_func}.

We start with part (a). By the definition of the optimization problem in \eref{gen_opt}, we have
\[
\Phi_{\mB}(\tau_1, \tau_2) \le \Phi_{\mB}(0, 0) + \tau_1 ([\wt_{\mB}]\tran \mSig \wt_{\mB}) + \tau_2 (\sqrt{p} \mu_1 \sgl\tran \fmtx \wt_{\mB})
\]
for any $\tau_1, \tau_2$. It follows that, for any $\tau > 0$,
\begin{equation}\label{eq:gen_bnds}
\frac{\Phi_{\mB}(\tau, 0) - \Phi_{\mB}(0, 0)}{p\tau} \le \genvar_B \le \frac{\Phi_{\mB}(-\tau, 0) - \Phi_{\mB}(0, 0)}{-p\tau}.
\end{equation}
Fix $\varepsilon > 0$. By Assumption~\ref{a:gen}, the limit function $q^\ast(\tau_1, \tau_2)$ is differentiable at the origin. Thus, there is some $\delta > 0$ such that
\[
\Big\vert\frac{q^\ast(\delta, 0) - q^\ast(0, 0)}{\delta} - \genvar^\ast\Big\vert \le \varepsilon / 3.
\]
The first inequality in \eref{gen_bnds}, with $\tau$ substituted by $\delta$, then gives us
\begin{align}
&\P(\genvar_B  - \genvar^\ast < -\varepsilon) \le \P\Big(\frac{\Phi_{\mB}(\delta, 0) - \Phi_{\mB}(0, 0)}{p\delta} - \genvar^\ast < -\varepsilon\Big)\nonumber\\
&\qquad\le \P(\absb{\Phi_{\mB}(\delta, 0)/p - q^\ast(\delta, 0)} > \delta \varepsilon / 3) \nonumber\\
&\hspace{6em}+ \P(\absb{\Phi_{\mB}(0, 0)/p - q^\ast(0, 0)} > \delta \varepsilon / 3).\label{eq:genvar_bnd}
\end{align}
By our assumption, $\Phi_{\mB}(\delta, 0)/p \cip q^\ast(\delta, 0)$ and $\Phi_{\mB}(0, 0)/p \cip q^\ast(0, 0)$. It then follows from \eref{genvar_bnd} that $\lim_{p \to \infty} \P(\genvar_B  - \genvar^\ast < -\varepsilon) = 0$. The same reasoning, applied to the second inequality in \eref{gen_bnds}, will give us $\lim_{p \to \infty} \P(\genvar_B  - \genvar^\ast > \varepsilon) = 0$, and thus $\genvar_B \cip \genvar^\ast$. The proof that $\gencor_B \cip \gencor^\ast$ is completely analogous and it is omitted.

Next, we move on to part (b) and establish the limits for $\genvar_A$ and $\gencor_A$. This is easy, in light of the universality laws given by Theorem~\ref{thm:get}. Specifically, \eref{get_cip} gives us $\Phi_{\mA}(\tau_1, \tau_2) / p \cip q^\ast(\tau_1, \tau_2)$. Replicating the same steps in part (a), with $B$ replaced by $A$, allows us to conclude that
\begin{equation}\label{eq:genA_sig_lim}
\genvar_A \cip \genvar^\ast \quad \text{and} \quad \gencor_A \cip \gencor^\ast.
\end{equation}
We can also show the function $G(\genvar, \gencor)$ is continuous at any point $(\genvar, \gencor)$ satisfying $\genvar \geq \gencor^2$ and $\rho\neq 0$. Let $z_1,z_2\iid \mathcal{N}(0,1)$ and $\{(\genvar_k,\gencor_k)\}_{k\geq 1}$ be a sequence converging to $(\genvar, \gencor)$, with $\genvar_k \geq \gencor_k^2$. Correspondingly, define $X_k:=[\fteacher(z_1) - \fout(\gencor_k z_1 + [{\genvar_k - \gencor^2_k}]^{1/2} z_2)]^2$ and $X:=[\fteacher(z_1) - \fout(\gencor z_1 + [{\genvar - \gencor^2}]^{1/2} z_2)]^2$. By Assumption \ref{a:fout}, $\fout$ is continuous almost everywhere, so if $\genvar \geq \gencor^2$ and $\rho\neq 0$, we can get $X_k\asconv X$, where $\asconv$ denotes almost sure convergence. On the other hand, since there exist some constants $C>0$ and $K_2\in\mathbb{Z}^+$ such that $\max\set{\abs{\fteacher(x)}, \abs{\fout(x)}} \le C(1 + \abs{x}^{K_2})$ by Assumption \ref{a:fout}, we have $|X_k|\leq C'(1+|z_1|^{2K_2}+|z_2|^{2K_2})$ for any $k\geq 1$, where $C'>0$ is a constant. Then by dominated convergence theorem, $G(\genvar_k, \gencor_k)=\E X_k \to \E X = G(\genvar, \gencor)$. This verifies the continuity of $G(\genvar, \gencor)$.
As a result,
\begin{equation}\label{eq:genAB_lim}
\gerrB \cip G(\genvar^\ast, \gencor^\ast) \quad \text{and} \quad G(\genvar_A, \gencor_A) \cip G(\genvar^\ast, \gencor^\ast).
\end{equation}

To complete the proof, we just need to establish part (c), namely, $\gerrA \approx G(\genvar_A, \gencor_A)$. To that end, we first write $\gerrA = \E_{\cvec_\text{new}}\btest(\scp \va_\text{new}\tran \wt_{\mA}, \cvec_\text{new}\tran \sgl)$, where
\[
\btest(x; s) \bydef (\fteacher(s) - \fout(x))^2.
\]
By Assumption~\ref{a:fout}, $\btest(x; s)$ is differentiable with respect to $x$ except at a finite number of points. Moreover, it is easy to check that
\[
\max\set{\abs{\btest(x; s)}, \abs{\btest'(x; s)}} \le C (1+\abs{s}^{2K_2})(1 + \abs{x}^{2K_2}),
\]
where $C > 0$ and $K_2\in \mathbb{Z}^+$ are the constants in Assumption~\ref{a:fout}. Our goal is to apply Proposition~\ref{prop:CLT_piecewise}, but we first need to put forth some additional restrictions. Let
\[
\mathcal{B} = \set{\norm{\wvv}_{\infty} \le \left(\log p\right)^{3+2K_{1}}},
\]
where $K_1$ is the constant in Assumption~\ref{a:loss} and
\[
\mathcal{C} = \set{\genvar_A = [\wt_{\mA}]\tran \mSig \wt_{\mA}/ p \ge \genvar^\ast/ 2}.
\]
Also recall the admissible set $\mathcal{A}$ defined in \sref{admissible}. We can verify that the assumptions of Proposition~\ref{prop:CLT_piecewise} (as stated and shown in \sref{CLT_disc}) hold for any $\fmtx \in \mathcal{A}$ and $\wvv = \wt_{\mA} \in \mathcal{B} \cap \mathcal{C}$. Thus, conditioned on $\mathcal{A} \cap \mathcal{B} \cap \mathcal{C}$, we can apply Proposition~\ref{prop:CLT_piecewise} to get
\begin{equation}\label{eq:gen_CLT}
\begin{aligned}
   &\abs{\E_{\cvec_\text{new}}\btest(\scp \va_\text{new}\tran \wt_{\mA}, \cvec_\text{new}\tran \sgl) - \E_{\cvec_\text{new}}\btest(\scp \vb_\text{new}\tran \wt_{\mA}, \cvec_\text{new}\tran \sgl)} \\
   \le& \frac{\polylog p}{p^{1/8}}. 
\end{aligned}
\end{equation}

Observe that $\E_{\cvec_\text{new}}\btest(\scp \vb_\text{new}\tran \wt_{\mA}, \cvec_\text{new}\tran \sgl) = G(\genvar_A, \gencor_A)$. Fix $\varepsilon > 0$.  For all sufficiently large $p$, we have ${\polylog p}/({p^{1/8}}) \le \varepsilon$. It then follows from \eref{gen_CLT} that
\begin{align}
&\P(\absb{\gerrA - G(\genvar_A, \gencor_A)} > \varepsilon) \nonumber \\
\le& \P(\mathcal{A}^c) + \P(\mathcal{B}^c) + \P(\mathcal{C}^c)\nonumber\\
\le& C e^{-C (\log p)^2} + \P(\absb{\genvar_A - \genvar^\ast} \ge \genvar^\ast / 2),\label{eq:genA_lim}
\end{align}
where to reach the last inequality we have used the probability estimates in \eref{A_small_prob} [for $\P(\mathcal{A}^c)$] and Lemma~\ref{lem:loowt_l_infty_bd} in Appendix~\ref{appendix:linfty_boundedness} [for $\P(\mathcal{B}^c)$]. Combining \eref{genA_lim}, \eref{genAB_lim}, and \eref{genA_sig_lim}, we complete the proof.

